Smaller Is Bigger: Rethinking the Embedding Rate of Deep Hiding

Deep hiding, concealing secret information using Deep Neural Networks (DNNs), can significantly increase the embedding rate and improve the efficiency of secret sharing. Existing works mainly force on designing DNNs with higher embedding rates or fancy functionalities. In this paper, we want to answer some fundamental questions: how to increase and what determines the embedding rate of deep hiding. To this end, we first propose a novel Local Deep Hiding (LDH) scheme that significantly increases the embedding rate by hiding large secret images into small local regions of cover images. Our scheme consists of three DNNs: hiding, locating, and revealing. We use the hiding network to convert a secret image in a small imperceptible compact secret code that is embedded into a random local region of a cover image. The locating network assists the revealing process by identifying the position of secret codes in the stego image, while the revealing network recovers all full-size secret images from these identified local regions. Our LDH achieves an extremely high embedding rate, i.e., $16\times24$ bpp and exhibits superior robustness to common image distortions. We also conduct comprehensive experiments to evaluate our scheme under various system settings. We further quantitatively analyze the trade-off between the embedding rate and image quality with different image restoration algorithms.

==> ieee copy/algorithm.tex <==
\section{Methodology}\label{sec:algorithm}
% \lhc{Due to the above vulnerabilities???}, we propose a Local Deep Hiding(LDH) architecture, embedding a full-size secret image into a random local region of arbitrary cover image with a hiding network, and recovering the original secret image with a revealing network.
% \lhc{Notation: $C,C',S,S_e,S',H,R,B',B$: cover image, stego image, secret image, encoded secret (i.e. noise), recovered secret image, hiding network, revealing network, predicted binary map, GT binary map}

\textbf{Insight.}
While surprised by the high embedding rate of deep hiding, we are also thinking about the reasons behind such improvement in the embedding rate and how to further improve it. By comparing traditional data hiding with deep hiding, we find that the encoding ability of DNNs is critical to improve the embedding rate since images are of high redundancy and DNNs can automatically embed secret image's information into the cover image without affecting its fidelity.
% In traditional data hiding \cite{chan2004hiding,pevny2010using,tamimi2013hiding,li2007steganographic,raja2005secure,mckeon2007strange}, all revealed secret information can only come from the corresponding secret codes.
% On the contrary, recent works of deep hiding \cite{baluja2017hiding,zhang2019invisible,zhang2020udh,yu2020attention,meng2019steganography,isola2017image,zhu2017unpaired,duan2019reversible} have show their advantage in achieving a high embedding rate (e.g., 24 bpp). \textit{What caused such a huge gap?} After analysis, we believe that the capacity of DNNs makes deep hiding have such a high embedding rate.

To demonstrate this phenomenon, we design a local embedding strategy to explain the working principle of deep hiding, which can also achieve a much higher embedding rate without affecting the visual quality of cover images. In particular, we propose a novel local deep hiding (LDH) method, where we convert a secret image into a small imperceptible compact code (e.g., the size of the code can be only $\frac{1}{16}$ of the secret image's size) using our hiding network. And we require the revealing network to recover the corresponding full-size and complete secret image. Obviously, the small imperceptible compact code carries the full information of the secret image and can be recognized by the revealing network, which is difficult for traditional data hiding due to their limited encoding ability. In addition, with the secret code becoming smaller, we can hide more images within different local regions of a cover image to improve the embedding rate by carefully designing the losses and the training process.

% the information carried by the small-scale code cannot support the complete recovery of the full-size image alone since a lot of information has been lost. The extra information required for the complete recovery can only come from the revealing network. Therefore, we can confirm that the revealing network does fit the redundant information of images. In addition, due to the local hiding strategy, we achieve multiple-image hiding for an unprecedented embedding rate (e.g., 16$\times$24 bpp).

% In our method, we aim to generate compact secret codes that have a much smaller size than secret images. At the same time, we still need to reveal the full-size secret images from small-scale secret codes. So, the revealing network must record the extra information beyond the secret codes to ensure the recovery of the complete and full-size secret images. Moreover, due to reduction of secret code size, we can hide much more secret images in a cover image simultaneously (i.e., a higher embedding rate than existing methods') since a secret image only occupies a small local region of the cover image.

% we reduce the scale of secret codes greatly and still require the network to reveal full-size secret images from the compact secret codes. With the reduction of the secret code scale, the network must remember extra image information besides the codes to ensure the recovery of the complete yet full-size images. In addition, based on the operation of reducing the scale of secret codes, we propose a novel locally embeddable multi-image hiding framework LDH to increase the embedding rate to an unprecedented level.


% In our framework, we encode different full-size secret images into very compact secret codes having much smaller size than the secret images and hide them into different small local regions of the cover image. In the revealing phase, we recover all full-size secret images from these local regions of the cover image.
% Intuition tells us that this is because the deep model has huge capacity and can remember some redundant secret information, which reduces the amount of information that needs to be encoded so the embedding rate increased. Therefore, as long as the network has enough capacity, we can achieve a higher embedding rate. To confirm it, we propose a novel deep hiding scheme that hides a full-size secret image into a local region of another one, and then reveals the secret image with its original size. In this way, we can achieve higher embedding rate by embedding different secret images into different regions in the cover image. Besides, the large-scale secret images are recovered from the small-scale coding results is enough to show that the decoder does remember the redundant information in images.

% Our LDH mainly starts from two directions, i.e., local embedding and rethinking of embedding rate. \emph{Firstly}, most of the existing deep hiding schemes hide the secret image of the same size as the cover image. However, the practical problem may not require this, such as embedding the secret image at a logo in a local region of the cover image. Thus, to break through the size limitation, our LDH allows local embedding by encoding the original secret image to a smaller perturbation. \emph{Secondly}, LDH enables local embedding, in other words we can embed multiple secret images into an identical cover image. Does this mean that the evaluation metrics such as \emph{bits-per-pixel (bpp)} are no longer applicable to evaluate the embedding rate of an image? We know that color images' each pixel contains 24 bits ($8\times(R, G, B)$), but if we embed 4 secret images into different local regions of 1 cover image at the same time, and all of them can be restored with an acceptable distortion, can we say that the embedding amount of this cover image achieves $4\times24$ bpp? Obviously, this is contradictory to the facts stated earlier. So it's of great necessity to design a method to quantify the result of encoding secret image and propose a new metric to measure the amount of information embedded.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/algorithm/pipeline.pdf}
%     \caption{The proposed LDH framework.}
%     \label{fig:pipeline}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/algorithm/pipeline.pdf}
    \caption{The proposed LDH framework.}
    \label{fig:pipeline}
    % \vspace{-10pt}
\end{figure*}

\textbf{Pipeline.} We illustrate the pipeline of the proposed LDH in Fig. \ref{fig:pipeline}, which consists of two modules: hiding and revealing module. \textit{In the hiding module,} we design a hiding network ($H$) to convert a given secret image ($S$) into a small imperceptible compact code ($S_e$), whose size is smaller than $S$. And then, we hide the compact secret code $S_e$ within a random local region of $C$ to produce the corresponding stego image ($C'$). Note that our method is  universal, where the same $S_e$ can be hidden into different cover images. \textit{In the revealing module,} there are two DNNs: locating and revealing networks. We first design a locating network $P$ to identify the position of $S_e$ in $C'$ by producing a binary map ($B'$). Next, we crop the determined local region of $C'$ according to $B'$ and feed the cropped result to a revealing network ($R$) to recover the corresponding full-size secret images ($S'$).


% no longer converts a given secret image ($S$) into a secret code ($S_e$) with the same scale as the $S$ for global embedding liking that in \cite{baluja2017hiding,zhang2020udh},
% but generates compact $S_e$  which has a smaller size than $S$. And we hide the compact $S_e$ within a random local region of a cover image ($C$) to get the corresponding stego image ($C'$). Similarly, we can hide other secret images in the remaining regions of $C$ to achieve multiple-image hiding.
% \textit{In the revealing module,} the locating module first identifies the position of each $S_e$ in $C'$ by producing a binary map. Then, we crop all determined local regions of $C'$ according to the binary map and feed them to the revealing
% \textit{In the locating phase,} $P$ takes $C'$ as its input and outputs a binary map ($B'$) to identify the locations of all embedded $S_e$ in $C'$. \textit{In the revealing phase,} we crop all determined local regions of $C'$ according to $B'$ and feed them to $R$ to recover the corresponding full-size $S'$.
% a hiding network ($H$), a locating network ($P$), and a revealing network ($R$).





% The \emph{Hiding (H)} network encodes the full-size secret image ($S$) to a smaller encoded image($S_e$), $S_e$ will be added to the local region of cover image ($C$) at random position to obtain the container image $C'$, then the \emph{detecting (D)} network plays a role in detecting $S_e$, revealing the location of $S_e$ through the generated map ($map$), which is used as auxiliary information to help \emph{Restoring (R)} network to notice $S_e$ and decode it to obtain the full-size restored image $S'$. Note that the input of \emph{R} is only a part of $C'$ that contains $S_e$. The overall training process is divided by two stages. Specifically, the $S_e$ used to restore the $S$ is generated by co-training \emph{H} and \emph{R} network at stage 1, when the training results of stage 1 is stabilizing, freeze \emph{H} and \emph{R}s' parameters and start the second stage of training. In stage 2, \emph{D} network only needs to train a few epochs to reach convergence and generate a map with location information, which will later assist \emph{R} in decoding and restoring.
% Both the $map$ used to determine the location of $S_e$ and the $S_e$ used to restore the $S$ are generated by co-training \emph{H}, \emph{D} and \emph{R} network.


\subsection{Networks for LDH}
\textbf{Hiding Network.} Existing deep hiding schemes \cite{baluja2017hiding,zhang2020udh,yu2020attention} usually conceal one or more secret image(s) within a cover image of the same size. However, since multiple secret image information is embedded into all pixels of the cover image, the robustness and the visual quality of the revealed secret images would be affected. Thus, it is difficult to increase the embedding rate of deep hiding in such a global manner. In addition, one cannot clearly figure out the working principle of deep hiding. To address the problems, we consider local embedding and design a novel hiding network to covert full-size secret images into small imperceptible compact codes as we have illustrated in Fig. \ref{fig:pipeline}.
% And the compact codes can be embedded into any local regions of the cover images through element-wise addition for hiding.
% At the same time, with the reduction of the size of secret codes, a cover image can carry more secret images by hiding the corresponding secret codes within different local regions of the cover image.

In the hiding network, we first adopt some down-sampling layers to reduce the scale of $S$, which are used to produce intermediate representations of $S$. And then, these intermediate representations are further encoded by $H$ that outputs the final small imperceptible compact secret code $S_e$. We use a scaling factor $\omega$ to control the size of $S_e$ in this paper, where $\omega$ is the ratio of the width of $S_e$ to the width of $S$. After obtaining $S_e$, we hide it within a random local region of a given cover image $C$ through element-wise addition as shown in Fig. \ref{fig:pipeline}. The complete hiding process can be formally represented as
\begin{equation}
    C'=Local\_Add(C,H(S, \omega)),
    \label{eq:local_add}
\end{equation}
where $Local\_Add$ denotes the addition operation. Please note that $\omega$ determines the upper bound of embedding rate.
% is related to the specific scaling factor adopted in experiments, as will be interpreted later.
% In experiments, we set the loss function of training $H$ as
% \begin{equation}
%     L_H = \|C-C'\|_2.
% \end{equation}

\textbf{Locating Network.} Since the small imperceptible code $S_e$ is embedded into $C$ locally and randomly, we need to identify the position of $S_e$ in $C'$. To this end, we design a locating network $P$ to automatically identify the regions that are embedded with $S_e$, which will assist the revealing network to reconstruct the secret image. The locating network $P$ takes $C'$ as its input and determines the position of $S_e$ in $C'$ by generating a binary map $B'$. In particular, we use 1 in $B'$ to indicate the corresponding pixel of $C'$ belongs to an embedding region and use 0 to indicate the opposite. The whole locating process is
\begin{equation}
    B'=P(C').
\end{equation}

% One of the advantages of using the locating network $P$ is to save computational resources. If $P$ is not used, the recovery process requires recovering and upsampling the entire $C'$ \lhc{??}, obtaining a large-size image containing a lot of useless redundant information, and finally cropping the correctly recovered region out. Obviously, this would result in a serious waste of computational resources. If a region containing secret information is located and cropped out beforehand, the subsequent recovery process only need to deal with this local region, avoiding unnecessary computing overhead.

% $P$ sets the value at the location considered to contain $S_e$ to 1, and sets the tensor value at the remaining locations to 0.
% The generated map $B'$ will be used as auxiliary information to assist the subsequent revealing process.

% and to train a satisfactory $P$, we try to minimize a loss function as
% % we transform the true location into a binary map $B'$ and compare it with the predicted map $B$, i.e., train $P$ by:
% \begin{equation}
%     L_P = \|B-B'\|_2,
% \end{equation}
% where $B$ represents the ground truth of binary maps.

\textbf{Revealing Network.} In previous works \cite{baluja2017hiding,zhang2019invisible,zhang2020udh,yu2020attention}, the revealing network recovers $S'$ from $S_e$ that has the same size as $S'$. Although these works achieve an embedding rate of 24 bpp or higher, they still do not fully exploit the potential of the revealing network. In LDH, we make full use of the capability of the revealing network to record extra image information besides $S_e$ in its parameters. So our revealing network can recover the full-size $S'$ from the small compact $S_e$. Specifically, in $R$, we use its bottom layers to pre-process $S_e$ for getting the corresponding intermediate representation while maintaining the size. Then, we use the top layers of $R$ to further convert the representation and increase its size gradually until meeting the original size of $S$.
% design the top layers of $R$, including several convolution layers and transposed convolution layers, to gradually increase the size of intermediate result while maintaining its internal details.
% refer existing revealing networks to construct the bottom layers of our $R$ and add some extra upsampling layers to build the top layers of $R$.
% We first employ the bottom layers to transform $S_e$ to an intermediate result while maintaining its size. Then, we take the top layers to further increase the size of representations of $S_e$ gradually until meeting the size of $S$.
The revealing process is summarized as
\begin{equation}
    S'=R(Cr(C',B')),
\end{equation}
where $Cr(C', B')$ means applying the cropping operation to $C'$ under the guidance of $B'$.

% In experiments, we use the technology of super-resolution (SR) reconstruction \cite{dong2016accelerating} to realize the top layers. Specifically, we initialize the top layers using pre-trained weights for SR tasks in our training. As discussed in Section \ref{sec:experimental_evaluation}, this way implicitly constrains the bottom layers of $R$ to recover secret images with small size even we do not constrain it explicitly in the loss function. \lhc{such detail description should be placed in experiments}

% , which is shown as
% The whole revealing process  which can be described as $S'=R(C',B')$.
% The revealing network has the heaviest task: revealing a full-size recovered secret image $S'$ from $C'$ that contains encoded information $S_e$ in only local region.
% To implement this function, we employ a dense convolutional layer for decoding the $S_e$ in the local area of $C'$ to learn more encoded information. Afterwards, several convolutional layers are needed for upsampling, aiming to reveal the full-size recovered secret image $S'$ from the locally decoded information, i.e. $S'=R(C',B')$. The loss function of this process can be expressed as:
% \begin{equation}
%     L_R = \|S-S'\|_2.
% \end{equation}
% The excellent performance of $R$ indicates that our LDH model has indeed learned a more compact representation with stronger capacity to further improve the embedding rate.


% \textbf{Module.} As shown in ***, our LDH consists of the three parts, \emph{H}, \emph{D} and \emph{R} network. CycleGAN is suitable for image-to-image translation tasks \cite{zhu2017unpaired, isola2017image}, hence \emph{H} is based on CycleGAN and adopts some simplifications. Specifically, \emph{H} network consists of several residual blocks which downsample and upsample the input sequentially, and in this process conduct skip connections to pass lower layers' feature to higher layers. Every residual block of \emph{H} network includes a convolution layer (kernel size = 4, stride = 2, padding = 1) and a transposed convolution layer (k = 4, s = 2, p = 1). Each convolution layer follows with an instance normalization layer and a LeakyReLU layer, and each transposed convolution layer applies ReLU activation function instead.

% As for \emph{D} network, due to the task of \emph{D} is lighter, it simply consists of several convolution layers (k = 3, s = 1, p = 1). First five convolution layers follow with an instance normalization layer and a ReLU layer, the last one follows with a sigmoid layer.

% \emph{R} network decode the input and rescale the result, adopting a dense CNN. Including six convolution layers (k = 3, s = 1, p = 1) which follow with an instance normalization layer and ReLU layer similarly as \emph{D} does. In addition, there are also one convolution layer (k = 5, s = 1, p = 2), one convolution layer (k = 1, s = 1, p = 0), four convolution layers (k = 3, s = 1, p = 1), and two convolution layers (k = 1, s = 1, p = 0), each of them follows with a PReLU layer. The last layer is a transposed convolution layer (k = 9, s = 4, p = 4, output padding = 3) to get the full size output.

\subsection{Training Details}
We co-train the three networks to ensure the imperceptibility and security of secret sharing. In particular, we have three goals: 1) minimize the negative impact of the hiding to cover images; 2) accurately identify the location of the embedded regions; 3) minimize the difference between the original and revealed secret images. In the following, we introduce three loss functions to achieve these goals.
% The location information of the embedded secret image is directly given to $R$. Then co-train the three networks $H$, $D$, and $R$. During training, the overall loss function consists of three loss items, including concealing loss, locating loss and revealing loss, which we will then introduce these losses in detail respectively.

\textbf{Hiding Loss.} We use the hiding loss ($L_H$) for restraining $H$, which ensures the imperceptibility of $S_e$. A common way to make $C'$ close to $C$ is minimizing the $L_p$ distance between $C'$ and $C$ \cite{baluja2017hiding,zhang2020udh}. Therefore, in our experiments, we set $L_H$ as
\begin{equation}
    L_H = \|C-C'\|_p.
\end{equation}

% \lhc{We can add extra items to enhance the quality??}

% constrain the result of the network $H$ which encodes the input stego image $C'$ as a scaled-down invisible perturbation $S_e$ according to the scaling factor and adds it to the local region of the cover image $C$ by element.

% \lhc{[old version:]} In order to keep the resulting stego image from being detected by steganalysis \lhc{in related works, anti-steganalysis needs special designed adversarial loss. So I suggest removing this part}, the invisibility of the encoded result $S_e$ should be maximized, i.e., to make $C$ and $C'$ as similar as possible. The loss item $L_H$ of this part is defined as follows,
% \begin{equation}
%     L_H = \|C-C'\|_p.
% \end{equation}

\textbf{Locating Loss.} The accuracy of identifying the location of the embedded regions is crucial for our scheme since it affects the final revealing result directly. Before the training of $P$, we record the real positions of all embedded secret code $S_e$ in a binary map $B$ (i.e., ground truth), where $B_{ij}$ is 1 if the corresponding pixel in $C'$ carries secret information, otherwise it is 0. During the training process, we optimize $P$ to reduce the locating loss ($L_P$) between ground truth and the predict map $B'$ of $P$ , i.e.,
\begin{equation}
    L_P = \|B-B'\|_p.
\end{equation}

% directly determines the effect of subsequent revealing process, so the locating process is crucial.
% During training, the random position where $S_e$ embedded in the concealing process is recorded as a binary map $B$, which is used as the ground truth of the locating network $P$'s output $B'$ (the region containing the secret information in the stego image $C'$ is set to 1 and the rest of the positions are set to 0). Using the $C'$ generated by $H$ as input, the locating network is trained to output a binary map $B'$ that is as similar as possible to $B$, as follows,
% \begin{equation}
%     L_P = \|B-B'\|_2,
% \end{equation}

\textbf{Revealing Loss.} $R$ is responsible for revealing $S'$ from the cropped stego image $C'$, which should be as close as possible to the original secret image $S$. Therefore, we also design the corresponding revealing loss ($L_R$) in the form of $L_p$-norm as
\begin{equation}
    L_R = \|S-S'\|_p.
\end{equation}



% During the revealing process, the revealing network should have the ability to recover the secret image with the original size with the assistance of the auxiliary information $B'$. Specifically, before the revealing process, $C'$ is first cropped according to $B'$ generated by the locating network, and then the result of the cropping is used as an input to the revealing network $R$ for recovery and super-resolution reconstruction to obtain the result $S'$. To obtain a high-quality $S'$, the revealing loss is defined as follows,
% \begin{equation}
%     L_R = \|S-S'\|_2.
% \end{equation}

With the above three loss items, we can obtain our final loss to training the three DNNs in our LDH, i.e.,
\begin{equation}
    L_T=\lambda_1 L_H + \lambda_2 L_P + \lambda_3 L_R,
\end{equation}
where $\lambda_1$, $\lambda_2$, $\lambda_3$ are three hyper-parameters.

\textbf{Training Strategy.} To better train the DNNs, we use a two-stage training strategy. Specifically, we split the whole training process into the pre-training and co-training phases. In the pre-training phase, we set $\lambda_2=0$. This is because, at the beginning of training, $P$ cannot determine the embedding regions correctly. We do not require $R$ to recover $S'$ from the non-embedding regions that would lead to a stagnation of training. Therefore, we do not consider $P$ in the pre-training phase. Note that, to train the $H$ and $R$, we use $B$ (the ground truth of locations) to crop $C'$ in this phase. After that, we start to co-train $H$, $P$, and $R$. Considering that $H$ and $R$ have been trained well, we focus primarily on training $P$ in the co-training phase. So we set $\lambda_2$ to a large value while $\lambda_1$ and $\lambda_2$ are small in the co-training.

% The accuracy of $P$ network of LDH depends heavily on the results of $H$, and the results of $P$ are crucial to the revealing process of $R$ similarly. Empirically, if the three networks are co-trained directly, it will lead to mutual constraints and training failure of them. Therefore, to reduce the blindness of training, we divided the overall training process into two phases, including a pre-training phase and a co-training phase.
% % As mentioned before, the pre-training phase trains the network $H$ and $R$.
% \emph{In the pre-training phase}, we aim at to obtain $H$ and $R$ with good performance. Specifically, during the pre-training, we crop $C'$ using the real locations of embedded secret images not using $B'$ generated by $P$. \emph{In the co-training}, we further train $H$, $R$, and $P$ jointly. Next, we will introduce how to complete the training in detail.

% As mentioned before, the complete training contains pre-training and co-training. In the pre-training, we only consider $H$ and $R$. And in the co-training, we train all three networks simultaneously. So the total loss ($L_T$) can be represented as
% % The total loss function consists of two stages of losses. To reduce the blindness of gradient descent, we first freeze the parameters of $P$ network and co-train $H$ and $R$ network. At this time, the $C'$ and the ground truth binary map $B$ are passed to the $R$ network, aiming to obtain a better pre-training result. We then co-train the $H$, $P$ and $R$ network, thus implementing the functions that the three networks should achieve. The overall loss function is shown in Eq. (\ref{eq:loss_overall})
% \begin{equation}
%     L_{T} =
%     \begin{cases}
%         \beta_1 L_H + \beta_2 L_R & \text{, pre-training} \\
%         \lambda_1 L_H + \lambda_2 L_P + \lambda_3 L_R & \text{, co-training}
%     \end{cases}
%     \label{eq:loss_overall}
% \end{equation}
% where $\beta_1$, $\beta_2$, $\lambda_1$, $\lambda_2$, $\lambda_3$ are hyperparameters that indicates the weight of each partial loss item. Moreover, in \cite{zhang2021brief}, $L_2$-norm is considered to be the most widely used loss function in deep learning based data hiding, it is sufficient to produce high-quality $C'$ and $S'$. So we also set $p=2$ for all individual loss items in experiments.

% \textbf{Loss Function.} As mentioned earlier, we co-train the three networks in two stages, and the scale and weight of them are totally different, with \emph{D} takes a lighter task than \emph{H} and \emph{R} do. $S_e$, the output of \emph{H}, will be added to $C$ and obtain $C'$, hence the loss of \emph{H} could be denoted as $\Vert C-C' \Vert_2$, so that make $S_e$ as invisible as possible. Similarly, \emph{R} takes charge of the restoration of $S$, consequently \emph{R} should minimize $\Vert S-S' \Vert_2$. As for \emph{D} in stage 2, its output $map$ provides an auxiliary position information for the restoration process of \emph{R}, so this loss can be expressed as the difference between $map$ and the true position, we denote it as $\Vert map-truth \Vert_2$. The overall error function can be described by below ($\beta_1, \beta_2$ are the weights of three different constituents):
% \begin{equation}
%     L_{Overall} =
%     \begin{cases}
%         \beta_1\Vert C-C' \Vert_2 + \beta_2\Vert S-S' \Vert_2& \text{, stage = 1} \\
%         \Vert map-truth \Vert_2& \text{, stage = 2}
%     \end{cases}
% \end{equation}

\subsection{Multiple Image Hiding}
Benefiting from the local embedding strategy, LDH enables multiple image hiding for a higher embedding rate. As shown in Fig. \ref{fig:diffpos}, four secret images are encoded as the corresponding imperceptible compact codes by $H$ and then embedded into different local regions of $C$. Note that our LDH can also support hiding multiple images into the same or overlapped local regions, which only requires to considering and adding this type of hiding samples into the ground truth during the training process. Without loss of generality, we only consider embedding multiple images into different regions of the cover image. Our locating network $P$ can identify all the positions of the embedded secret images and outputs a binary map containing multiple white areas. Finally, $R$ recovers all full-size secret images from the corresponding cropped regions of $C'$.
% all cropped local regions of $C'$ will be delivered to $R$ for recovering the corresponding full-size secret images.
% then these perturbations are sent to $P$ network which detects the locations of them. Finally, the stego image and the location information will be delivered to $R$ network for decoding and restoring.

Theoretically, \textit{LDH can support up to $\omega^2$ secret images (i.e., $\omega^2 \times 24$ bpp) simultaneously} if the communication parties agree on the value of $\omega$ in advance. And different from existing multi-image hiding schemes (e.g., UDH \cite{zhang2020udh}), LDH can conceal multiple images using onle one set of $H$, $R$, and $P$, not to train multiple network pairs. Thus, our LDH is more efficient. The multiple image hiding in LDH can be represented as
\begin{equation}
    C'=Local\_Add \left (C,\{H(S^{(k)}, \omega)\} \right ),
\end{equation}
where $S^{(k)}$ is the $k$-th secret image. And the corresponding revealing process is
\begin{equation}
    \{S'^{(k)}\}=R(Cr(C', P(C'))).
\end{equation}
% , LDH can achieve embedding up to 16 secret images ($16\times24$ bpp) simultaneously.
% In addition, unlike existing multi-image hiding schemes \cite{lu2021large,guan2022deepmih}, the recovery quality of LDH is not affected by the number of embedded secret images, as long as the number does not exceed the upper limit of what the network can accommodate (i.e., the squared number of the scaling factor). This is because LDH's $P$ network can accurately detect the locations of all embedded secret images in order to recover each secret image without interfering with each other. What's more, we realize the multi-image hiding using a set of $H$, $R$, and $P$, not training multiple pairs of $H$ and $R$ liking that in \cite{zhang2020udh}, which is more efficient.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/experiment/diffpos.pdf}
%     \caption{Concealing four different $S$ into the different positions of one $C$ using our LDH. All secret images could be detected and recovered in a high quality.}
%     \label{fig:diffpos}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/experiment/diffpos.pdf}
    \caption{Concealing four different $S$ into the different positions of one $C$ using our LDH. All secret images could be detected and recovered in high quality.}
    \label{fig:diffpos}
    \vspace{-10pt}
\end{figure}

% \lhc{the following description is unreasonable. remove, including Fig \ref{fig:multi_hiding}}
% \lhc{Taking the example of hiding two secret images, Fig. \ref{fig:multi_hiding} shows two ways of multiple image hiding. According to different application scenarios, LDH can either hide multiple secret images at the same time or hide secret images separately in multiple stages. In the first method, the hiding process can be formulated as
% \begin{equation}
%     C'=Local\_Add(C, H(S_1), \cdots, H(S_n))
% \end{equation}
% also, the hiding process of the second method can be formulated as
% \begin{equation}
%     C_i^{'} =
%     \begin{cases}
%         Local\_Add(C, H(S_1)) & , i=1\\
%         Local\_Add(C_{i-1}^{'}, H(S_i)) & , i>1
%     \end{cases}
% \end{equation}
% where the last $C^{'}_{i}$ is the final stego image $C'$. Compared to the first method, the second method is more applicable to the scenario of multiple users with embedding requirements. What's more, no matter which way the images are hidden in, the locating and revealing process of LDH is identical without adding additional training.}

% \begin{figure}[htbp]
%     \centering
%     \subfloat[]{\includegraphics[width=0.95\linewidth]{figs/algorithm/sub1.pdf}}
%     \quad
%     \subfloat[]{\includegraphics[width=0.95\linewidth]{figs/algorithm/sub2.pdf}}
%     \caption{Two methods of multiple image hiding. (a) indicates embedding multiple $S$ into $C$ at the same time, and (b) indicates embedding $S$ in multiple stages separately, and the stego image $C'$ of the previous stage is used as the cover image $C$ of the next stage.}
%     \label{fig:multi_hiding}
% \end{figure}

In addition to significantly increase the embedding rate, LDH has another advantage: LDH can further reduce the risk of being detected the existence of the sharing secrets by embedding $S_e$ within texture-rich local regions of $C$. For example, one can use the Just Noticeable Difference \cite{wu2017enhanced} (JND) technique to measure the human eye's sensitivity to distortion in different regions and find the most suitable positions for concealing secret images, which would obtain a $C'$ with better visual quality.

% In practical scenarios where data hiding is required, it is often not necessary to embed the secret image into the entire cover image, and LDH is well suited for such scenarios \lhc{???}. The cover image $C$ used as the embedding medium is often not a homogeneous image, with some regions having rich details and complex textures, and others having simple and plain smooth textures. The choice of the location of the embedded local region has a great impact on the visual quality of the generated stego image $C'$. For example, using JND \cite{wu2017enhanced} (Just Noticeable Difference) can find a most suitable location for embedding, minimizing the changes caused by embedding secret images. Note that the embedding location found using the JND method can make the changes before and after embedding more difficult for the human eye to notice, but does not change the metrics such as the PSNR of the $C$/$C'$ and the $S$/$S'$ image pairs.

==> ieee copy/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we propose a local deep hiding (LDH) scheme to demonstrate the reason behind the success of deep hiding at improving the embedding rate. LDH converts a secret image into a small imperceptible compact code using our hiding network and embeds the code into a random region of a cover image. The secret image can be revealed with a high quality using the locating and revealing network. Our extensive experiments have shown that the proposed method not only has a high embedding rate, but also achieves stronger robustness than existing deep hiding schemes. We also analyze the impact of different image restoration algorithms on the embedding rates of different deep hiding schemes.


==> ieee copy/embedding_rate_analysis.tex <==
\section{Embedding Rate Analysis}
\label{sec:embedding_analysis}
Data hiding can be viewed as a 2-player game, in which the sender embeds secret messages into a cover image, and the receiver recovers the secret messages from the stego image. As we have discussed in Table \ref{table:diff_scale}, the quality of revealed images is crucial in data hiding since serious distortions make the hiding meaningless. In this section, we discuss the embedding rate from the perspective of the receiver.

% In order to explore the embedding rate under different deep hiding schemes, we conduct the following experiments from the receiver's perspective.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/analysis/udh-ddh-mis-weng-multi.pdf}
    \caption{Recovered examples of DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh}, HCVS \cite{weng2019high} and MISDNN \cite{das2021multi} (from left to right) when hiding multiple images. The first row shows the revealed secret images and the second row shows the enlarged version of the regions in the boxes.}
    \label{fig:udh_ddh_multi}
\end{figure}

During the evaluation experiments, we find that the distortions on the recovery secret images (see Fig. \ref{fig:udh_ddh_multi}) are pattern-specific such as undesired stripe textures, the outline textures of $C$, and color distortion. These distortions may be reduced or even eliminated using extra image restoration algorithms. Therefore, we consider various receivers with different capacities to discuss the upper bound of the embedding rate of different deep hiding schemes. Specifically, we consider that the receiver can use non-learning-based algorithms or learning-based algorithms to further process the revealed secret images. Besides, it is necessary to set a threshold for the quality of recovered secret images to discuss the embedding rate. We set the the final embedding rate of a deep hiding scheme is the highest embedding rate that can be achieved when a specific scheme can meet this threshold.



% of DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh}, Weng et al. \cite{weng2019high} and MISDNN \cite{das2021multi}, including some stripe textures, the outline textures of $C$ and color distortion as shown in . These distortions can be reduced or eliminated by existing methods. To verify the superiority of our LDH in terms of embedding rate from the receiver's perspective, we consider giving the other hiding schemes' receivers various capabilities to further enhance the visual quality of the revealed results after decoding and revealing.

% Next, we record the highest embedding rate that can be achieved by each scheme when the average quality of the recovered images from these schemes exceeds a certain threshold. In our experiments, we use some non-learning-based algorithms and learning-based algorithms as the low-capability and high-capability algorithms, respectively, to enhance the visual quality of the recovered results, as shown below.

\textbf{Receiver with Non-learning-based Algorithms.} We assume that the receiver can take some non-learning-based image enhancement or denoising algorithms to further process the recovered images here. These algorithms are usually light and easy to implement, which do not require the receiver to have expensive computing and data resources. The experimental results of different schemes are recorded in Table \ref{table:low} when we set the threshold as 32 dB.

% which usually rely on some specific theories, such as histogram equalization \cite{ibrahim2007brightness}, retinex \cite{lee2013adaptive} and so on.
%  These methods are more lightweight and easy to implement, so we consider these methods as low-capability algorithms of the receiver in the experiments. The enhancement of the recovery results by these methods is small, we record the highest embedding rates of different hiding schemes when the PSNR of the recovered $S'$ is greater than 32dB, as shown in the Table \ref{table:low}. It can be seen that our LDH performs much better.

\begin{table}[t]
    \centering
    \caption{The embedding rate of different schemes when the receiver owns non-learning-based image restoration algorithms. The threshold is 32 dB.}
    \label{table:low}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    Method & BPDHE \cite{ibrahim2007brightness} & AMSR \cite{lee2013adaptive}  & LIME \cite{guo2016lime}  & NLFMT \cite{shreyamsha2013image}  & None  \\
    \hline
    DDH \cite{baluja2017hiding}         & 3$\times$24  & 3$\times$24  & 3$\times$24  & 3$\times$24  & 3$\times$24   \\
    UDH \cite{zhang2020udh}             & 2$\times$24  & 2$\times$24  & 2$\times$24  & 2$\times$24  & 2$\times$24   \\
    MISDNN \cite{das2021multi}          & 1$\times$24  & 1$\times$24  & 1$\times$24  & 1$\times$24  & 1$\times$24   \\
    HCVS \cite{weng2019high}     & 3$\times$24  & 3$\times$24  & 3$\times$24  & 3$\times$24  & 3$\times$24   \\
    LDH   & 16$\times$24 & 16$\times$24 & 16$\times$24 & 16$\times$24 & 16$\times$24  \\
    \bottomrule
    \end{tabular}
    }
\end{table}

\textbf{Receiver with Learning-based Algorithms.} A receiver may own expensive computing and data resources such that he can train a powerful image restoration model to enhance the image quality of the revealed secret images. In this experiment, we consider two state-of-the-art image restoration models: Restormer \cite{zamir2022restormer} and MPRNet \cite{zamir2021multi}, and train them respectively for different hiding schemes. We show the embedding rate of a high-capability receiver in Table \ref{table:middle-high}.

From both Table \ref{table:low} and \ref{table:middle-high}, we observe that the receiver with non-learning-based algorithms cannot increase the embedding rates of the involved schemes, while the receiver with learning-based algorithms can improve the quality of the secret images of the baselines, where Restomer is effective for both the lower and higher thresholds and MPRNet is effective for the lower threshold.
Our LDH has obvious advantages in terms of the embedding rates that are very high and are not affected by the receivers with different image restoration methods. The experimental results show that the involved baselines cannot hide more than 6 images when the threshold is larger than 26 dB, while our LDH can hide 64 images.
%  Such a great gap fully demonstrates the progressiveness of the idea of local hiding.

% For each group of DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh}, Weng et al. \cite{weng2019high} and MISDNN \cite{das2021multi} with different embedding rates, we save the recovered $S'$ and the original $S$ in pairs and randomly select 1000 image pairs as the dataset to fine-tune these mentioned restoration models. According to the general settings of image restoration, we use the original $S$ as the high quality ground truth and the recovered $S'$ as the low quality input.

% For comparison, we first determined two thresholds (26dB and 32dB) using the average PSNR scores of our LDH at scaling factors of 8 and 4 respectively. Subsequently, we gradually increase the number of other hiding schemes embedded images,  and use the above algorithms to improve the quality of recovered results $S'$. Finally, record the highest embedding rate that can be achieved when the recovery quality of other hiding schemes exceeds the set thresholds. The final results are shown in Table \ref{table:middle-high}. From this table, we can see the superiority of our LDH in embedding rate. All other hiding schemes obtain severely corrupted recovery results when embedding more than 6 images. With the identical expected recovery quality, the highest embedding rate that our LDH can achieve far exceeds that of other hiding schemes. Besides, we also find that the quality of the stego image $C'$ obtained by other hiding schemes degrades severely when embedding multiple secret images (this is also reflected in Fig. \ref{fig:stego_quality}), which is against the expectation of deep hiding.

\begin{table}[t]
    \centering
    \caption{The embedding rate of different schemes when the receiver owns learning-based image restoration algorithms.}
    \label{table:middle-high}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{PSNR$\geq$26dB} & \multicolumn{3}{c}{PSNR$\geq$32dB}  \\
        \cline{2-7}
                                & Restomer & MPRNet & None             & Restomer & MPRNet & None             \\
        \hline
        DDH \cite{baluja2017hiding}     & 6$\times$24     & 5$\times$24 & 5$\times$24               & 4$\times$24     & 3$\times$24 & 3$\times$24               \\
        UDH \cite{zhang2020udh}         & 5$\times$24     & 4$\times$24 & 3$\times$24               & 3$\times$24     & 2$\times$24 & 2$\times$24               \\
        MISDNN \cite{das2021multi}      & 4$\times$24     & 3$\times$24 & 2$\times$24               & 1$\times$24     & 1$\times$24 & 1$\times$24               \\
        HCVS \cite{weng2019high} & 6$\times$24     & 5$\times$24 & 5$\times$24               & 4$\times$24     & 3$\times$24 & 3$\times$24               \\
        LDH                     & 64$\times$24    & 64$\times$24 & 64$\times$24              & 16$\times$24    & 16$\times$24 & 16$\times$24              \\
        \bottomrule
    \end{tabular}
    }
\end{table}



==> ieee copy/experimental_evaluation.tex <==
\section{Experiments}\label{sec:experimental_evaluation}

\subsection{Configurations}
\textbf{Dataset.} We use ImageNet and COCO to evaluate all involved hiding schemes \cite{baluja2017hiding,zhang2020udh,yu2020attention,lu2021large,guan2022deepmih}. For each dataset, we randomly select 10,000 images, including 8,000 for training, 1,000 for validation and 1,000 for testing. All selected images are resized to $1024\times1024$, and pixel values are normalized within $\left [ 0, 1 \right ]$.

\textbf{Implementation of LDH and Baselines.}
In the implementation of LDH, we first consider $\omega=4$ (i.e., the size of $S_e$ outputted by $H$ is $256\times256$), and we discuss other values of $\omega$ in later subsection. For $H$, we adopt a convolution layer and a max pooling layer to build its shallow layers for acquiring small-size features maps. Then, we adopt UNet \cite{ronneberger2015u} to build its remaining layers, which is responsible for generating small-size yet imperceptible secret codes, i.e., compact codes $S_e$. To produce the binary map, we design the network $P$ as a full-convolution network with six convolution layers, which keeps the size of its input and output consistent. As for the network $R$, we also use six convolution layers to build its shallow layers for preprocessing its inputs, and we take the network proposed in \cite{dong2016accelerating} to gradually increase the size of feature maps until meeting the size of the original secret images. As described in the previous section, in the pre-training phase, we set $\lambda_1=0.25$, $\lambda_2=0$, and $\lambda_3=0.75$ to obtain a well-trained $H$ and $R$. In the co-training phase, the main goal is to train $P$ that can accurately locate the position of $S_e$, so we set $\lambda_1=0.1$, $\lambda_2=0.8$ and $\lambda_3=0.1$. Besides, we set the initial learning rate to 0.001 and scale it down by a factor of 0.1 after every 30 epochs during the training process. All networks are trained with the Adam optimizer \cite{kingma2014adam}.

We also consider some baselines for comparison, including DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh}, HCVS \cite{weng2019high} and MISDNN \cite{das2021multi}. We follow the public-available implementations\footnote{https://github.com/arnoweng/PyTorch-Deep-Image-Steganography}$^,$\footnote{https://github.com/ChaoningZhang/Universal-Deep-Hiding}$^,$\footnote{https://github.com/muziyongshixin/pytorch-Deep-Steganography}$^,$\footnote{https://github.com/m607stars/MultiImageSteganography} to implement the four baselines respectively. We also achieve multiple-image hiding for DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh}, and HCVS \cite{weng2019high} by concatenating multiple secret images in the channel dimension. For MISDNN \cite{das2021multi}, we adjust the embedding rate by increasing or decreasing the number of network pairs.
\begin{table*}[t]
    \centering
    \caption{Performance comparison. $\uparrow$ denotes higher value is better, and vice versa.}
    \label{table:performance}
    \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{|c|ccc|ccc|ccc|ccc|}
            \hline
            \multirow{3}{*}{Method}                         & \multicolumn{6}{c|}{Cover/Stogo 1 pair}                   & \multicolumn{6}{c|}{Secret/Recovery 1 pair}                \\
            \cline{2-13}
                                                            & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO}  \\
            \cline{2-13}
                                                            & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$     & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$      \\
            \hline
            DDH \cite{baluja2017hiding}     & 2.552  & 0.961 & 37.963       & 2.417  & 0.978 & 37.942   & 2.261  & 0.991  & 39.055      & 1.956  & 0.989 & 39.614    \\
            UDH \cite{zhang2020udh}         & 2.031  & 0.979 & 40.035       & 2.121  & 0.981 & 39.746   & 2.850  & 0.969  & 35.796      & 2.694  & 0.975 & 36.708    \\
            MISDNN \cite{das2021multi}      & 2.607  & 0.974 & 37.413       & 2.411  & 0.980 & 37.780   & 4.309  & 0.970  & 33.065      & 4.301  & 0.969 & 33.146    \\
            HCVS \cite{weng2019high} & 2.566  & 0.955 & 37.571       & 2.531  & 0.961 & 37.763   & 2.243  & 0.989  & 39.032      & 2.253  & 0.982 & 38.978    \\
            Ours                            & 0.346  & 0.994 & 43.887       & 0.292  & 0.996 & 45.118   & 3.809  & 0.951  & 33.169      & 3.974  & 0.947 & 32.963    \\
            \hline
            \hline
            \multirow{3}{*}{Method}         & \multicolumn{6}{c|}{Cover/Stogo 2 pairs}                   & \multicolumn{6}{c|}{Secret/Recovery 2 pairs}                \\
            \cline{2-13}
                                            & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO}  \\
            \cline{2-13}
                                            & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$     & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$      \\
            \hline
            DDH \cite{baluja2017hiding}     & 3.165  & 0.964  & 36.150      & 3.179  & 0.964 & 35.815   & 3.190  & 0.984  & 35.960      & 3.128  & 0.982 & 35.812    \\
            UDH \cite{zhang2020udh}         & 3.398  & 0.954  & 35.940      & 3.376  & 0.953 & 36.006   & 4.632  & 0.953  & 32.435      & 4.502  & 0.956 & 32.846    \\
            MISDNN \cite{das2021multi}      & 6.479  & 0.935  & 30.086      & 6.040  & 0.936 & 30.177   & 7.035  & 0.934  & 29.089      & 7.046  & 0.931 & 28.940    \\
            HCVS. \cite{weng2019high} & 3.688  & 0.953  & 34.839      & 3.808  & 0.953 & 34.331   & 3.467  & 0.977  & 35.412      & 3.517  & 0.968 & 35.092    \\
            Ours                            & 0.657  & 0.987  & 41.188      & 0.572  & 0.989 & 42.185   & 3.809  & 0.951  & 33.169      & 3.974  & 0.947 & 32.963    \\
            \hline
            \hline
            \multirow{3}{*}{Method}         & \multicolumn{6}{c|}{Cover/Stogo 3 pairs}                   & \multicolumn{6}{c|}{Secret/Recovery 3 pairs}                \\
            \cline{2-13}
                                            & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO}  \\
            \cline{2-13}
                                            & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$     & APD$\downarrow$    & SSIM$\uparrow$   & PSNR$\uparrow$        & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$      \\
            \hline
            DDH \cite{baluja2017hiding}     & 4.160  & 0.940  & 33.824        & 4.270  & 0.937 & 33.641   & 3.806   & 0.978 & 34.391      & 3.846  & 0.978  & 34.340   \\
            UDH \cite{zhang2020udh}         & 4.120  & 0.933  & 34.392        & 4.145  & 0.935 & 34.336   & 6.430   & 0.936 & 30.321      & 6.110  & 0.932  & 30.375   \\
            MISDNN \cite{das2021multi}      & 11.102 & 0.886  & 25.694        & 9.647  & 0.893 & 26.407   & 10.708  & 0.892 & 25.682      & 10.17  & 0.903  & 25.957   \\
            HCVS \cite{weng2019high} & 5.080  & 0.912  & 32.301        & 5.056  & 0.930 & 32.177   & 3.802   & 0.971 & 34.616      & 3.871  & 0.965  & 34.130   \\
            Ours                            & 0.983  & 0.982  & 39.572        & 0.988  & 0.984 & 39.651   & 3.809   & 0.951 & 33.169      & 3.974  & 0.947  & 32.963   \\
            \hline
            \hline
            \multirow{3}{*}{Method}         & \multicolumn{6}{c|}{Cover/Stogo 4 pairs}                   & \multicolumn{6}{c|}{Secret/Recovery 4 pairs}                \\
            \cline{2-13}
                                            & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c|}{COCO}  \\
            \cline{2-13}
                                            & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$         & APD$\downarrow$   & SSIM$\uparrow$   & PSNR$\uparrow$     & APD$\downarrow$    & SSIM$\uparrow$   & PSNR$\uparrow$        & APD$\downarrow$    & SSIM$\uparrow$   & PSNR$\uparrow$     \\
            \hline
            DDH \cite{baluja2017hiding}     & 5.758  & 0.927 & 31.118       & 5.611  & 0.923 & 31.147   & 6.679   & 0.964 & 29.909      & 6.440   & 0.962  & 30.061  \\
            UDH \cite{zhang2020udh}         & 4.740  & 0.915 & 33.163       & 4.755  & 0.917 & 33.139   & 10.785  & 0.891 & 25.725      & 10.414  & 0.882  & 25.767  \\
            MISDNN \cite{das2021multi}      & 16.38  & 0.823 & 21.797       & 18.38  & 0.817 & 20.862   & 13.667  & 0.841 & 23.243      & 12.117  & 0.855  & 24.095  \\
            HCVS \cite{weng2019high} & 5.076  & 0.919 & 31.948       & 5.331  & 0.921 & 31.803   & 6.806   & 0.947 & 29.505      & 6.817   & 0.955  & 29.990  \\
            Ours                            & 1.377  & 0.974 & 37.901       & 1.140  & 0.983 & 39.283   & 3.809   & 0.951 & 33.169      & 3.974   & 0.947  & 32.963  \\
            \hline
        \end{tabular}
    }
\end{table*}


\textbf{Evaluation Metrics.} To quantify the performance of all involved schemes, we use three visual metrics to measure the distance between $C$ and $C'$ (or $S$ and $S'$), including Average Pixel Discrepancy (APD), Peak Signal-to-Noise Ratio (PSNR), and Structural Similarity Index (SSIM).
% To evaluate the performance of the proposed model and to quantify the quality of the images generated by the concealing and revealing processes, we used three metrics to measure the quality of $C'$ relative to $C$ and $S'$ image relative to $S$, including Average Pixel Discrepancy (APD), Structural Similarity Index (SSIM), and Peak Signal-to-Noise Ratio (PSNR). The formulaic description of the three metrics is shown below.
\begin{itemize}
    \item \textbf{APD}. APD is the average $L_1$-norm distance between images, which can be formulated as
    \begin{equation}
        APD=\frac{1}{WH}\sum_{i=1}^{W}\sum_{j=1}^{H}\left | I_{i,j}-K_{i,j} \right |,
    \end{equation}
    where $I$ and $K$ are the reference image ($C$ or $S$) and the corresponding distorted image ($C'$ or $S'$) respectively. $H$ and $W$ are the height and width of images. The coordinate $(i,j)$ reflects the position of pixel $I_{i,j}$ (or $K_{i,j}$).
    % with width $W$ and height $H$
    % where $I_{i,j}$ and $K_{i,j}$ indicate the pixel values at position $[i,j]$ of images $I$ and $K$, respectively.

    \item \textbf{PSNR}. PSNR is a popular metric used to quantify the quality of signal reconstruction and is wildly used in related study. It is constructed based on $L_2$-norm as
    % It is often used as a measure of signal reconstruction quality in vision domain, and it is often defined simply by mean square error (MES). Since the direct use of MSE may have a very wide dynamic range, the PSNR is often expressed as a logarithmic quantity using the decibel scale. The formula for PSNR is shown as follows:
    \begin{equation}
            PSNR = 10\cdot\log_{10}{\left ( \frac{MAX_I^2}{MSE} \right )},
    \end{equation}
    where
    \begin{equation}
        MSE = \frac{1}{WH}\sum_{i=1}^{W}\sum_{j=1}^{H}\left [ I_{i,j}-K_{i,j} \right ]^2,
    \end{equation}
    and $MAX_I$ indicates the maximum possible pixel value of the image, which is 1 in experiments.

    \item \textbf{SSIM}. SSIM measures the similarity between two images mainly based on the perceived change in structural information. It is also commonly used in related studies, which can be represented as
    %  reflects the degree of similarity between two digital images. Given two images $x$ and $y$, SSIM can be calculated as follows:
    \begin{equation}
        SSIM=\frac{(2\mu_I\mu_K+c_1)(2\sigma_{IK}+c_2)}{(\mu_I^2+\mu_K^2+c_1)(\sigma_I^2+\sigma_K^2+c_2)}
    \end{equation}
    where $\mu_I$ (or $\mu_K$) is the mean values of $I$ (or $K$), $\sigma_I$ (or $\sigma_K$) the variances of $I$ (or $K$), and $\sigma_{IK}$ is the covariance between $I$ and $K$. $c_1$ and $c_2$ are used to maintain stability, where $c_1=(k_1L)^2$ and $c_2=(k_2L)^2$. $L$ has the same meaning as $MAX_I$. By default, we set $k_1=0.01$ and $k_2=0.03$.    % and $L$ is the dynamic range of pixel values. The default value of $k_1$ is 0.01 and $k_2$ is 0.03.
\end{itemize}
% These three metrics are calculated using the generated images and the corresponding original images.
The smaller the APD value, or the larger the PSNR and SSIM values, the better the quality of the generated image, meaning better hiding or revealing performance.

% \begin{longtable}{cccc}
%     \caption{Performance comparison between DDH, UDH and our LDH}
%     \label{table:performance}\\
%     \toprule
%     Errors & PSNR & SSIM & APD\\
%     % &  &
%     \midrule
%     \endfirsthead
%     \multicolumn{4}{r}{table continue}\\
%     \toprule
%     Errors & PSNR & SSIM & APD\\
%     % & DDH $C$ & DDH $S$ & UDH $C$ & UDH $S$ & LDH $C$ & LDH $S$\\
%     \midrule
%     \endhead
%     \bottomrule
%     \multicolumn{4}{c}{table continue}\\
%     \endfoot
%     \bottomrule
%     \endlastfoot
%     DDH $C$ & 35.87 & 0.977 & 2.68\\
%     UDH $C$ & 38.13 & 0.968 & 2.36\\
%     LDH $C$ & 44.85 & 0.996 & 0.28\\
%     DDH $S$ & 34.72 & 0.981 & 3.50\\
%     UDH $S$ & 35.66 & 0.967 & 3.27\\
%     LDH $S$ & 33.16 & 0.936 & 4.40
% \end{longtable}

% \textbf{Baselines.}

% \begin{table}
%     \centering
%     \caption{Performance comparison between DDH, UDH and our LDH.}
%     \label{table:performance}
%     \begin{tabular}{@{}cccc@{}}
%         \toprule
%         Errors & PSNR & SSIM & APD\\
%         \midrule
%         DDH $C$ & 35.87 & 0.977 & 2.68\\
%         UDH $C$ & 38.13 & 0.968 & 2.36\\
%         LDH $C$ & 44.85 & 0.996 & 0.28\\
%         DDH $S$ & 34.72 & 0.981 & 3.50\\
%         UDH $S$ & 35.66 & 0.967 & 3.27\\
%         LDH $S$ & 33.16 & 0.936 & 4.40\\
%         \bottomrule
%     \end{tabular}
% \end{table}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/experiment/baseline.pdf}
    \caption{Visualization examples of hiding four secret images in one cover image. The first two images in the top row are the original cover image and the corresponding enlarged version of the region in red box, respectively. The remaining images in the top row are the revealed images and the enlarged local areas. From the second row to the bottom row, images in the odd columns are the enlarged local areas of the stego or revealed secret images produced by the marked hiding schemes, and images in the even columns are the difference images between the stego and cover images (or the revealed secret and original secret images). To facilitate observation, pixel values in each shown difference image are scaled by 7.}
    \label{fig:examples}
\end{figure*}


\subsection{Overall Evaluation}
\textbf{Quantitative Results.}
% We first evaluate the performance of our LDH with a scaling factor of 4 (same for qualitative results).
We evaluate all the involved schemes to hide 1, 2, 3 and 4 secret images within a cover image, and show the numerical results in Table \ref{table:performance}. From Table \ref{table:performance}, we can observe that our LDH performs much better than baselines in the hiding phase where the quality of $C'$ generated by LDH is best on all three metrics. With the compact secret codes, LDH can maintain the quality of $C'$ at a much high level (PNSR $>$ 37 dB) even after hiding up to 4 full-size secret images within a cover image.

For the revealing phase, LDH also shows its superiority. As one can observe from Table \ref{table:performance}, the quality of $S'$ does not be affected by the number of secret images in LDH. Instead, these baselines is not suitable for embedding more images because the quality of the secrets decreases as the number of the embedded secrets increase. The main reason for this gap between LDH and the baselines is that the hiding and revealing process of each secret image in LDH is independent. Thus, the revealing of different secret images will not affect each other, but the the multiple-image hiding of the baselines would cause mutual influence between channels. In the case of only hiding one secret image, the revealing quality of LDH is slightly lower than DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh} and HCVS \cite{weng2019high}, but similar with that of MISDNN \cite{das2021multi}. We think this is due to the fact that the compact secret codes cause the loss of some secret information compared with the full-size imperceptible secret codes.

%  This problem can be alleviated by adopting some image restoration networks as we will discuss in Section \ref{sec:embedding_analysis}.

% This benefits from the local embedding strategy. In LDH, the hiding and revealing processes of different secret images are independent and the secret codes of different secret images do not affect each other. However, in other schemes, the hiding and revealing of different secret images are non-independent and the secret codes of different secret images will overlap each other since all these models adopt global embedding strategy. And as the number of secret images increases, the negative impact of such overlap will become more prominent.
% Thus, the quality of $S'$ decreases (even PSNR $<$ 27 dB) as the number of secret images increases in other schemes. In the case of hiding one secret image, the recovery quality of LDH is slightly lower than DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh} and Weng et al. \cite{weng2019high}, but similar with that of another multiple image hiding model MISDNN \cite{das2021multi}. We think this is due to the fact that even if the hiding network of LDH encodes $S$ into a highly condensed representation, a part of details is still unavoidably lost during the down-sampling operation and this would be eliminated by adopting more powerful super-resolution reconstruction networks.

% \lhc{the reason of why the quality of $S'$ in LDH is lower when only hiding one secret image should be revised. And it is better to introduce the disadvantage after the description of advantage. you can create a new command for yourself liking ``lhc'' or ``guo'' (see the main.tex), and use it when you are not sure whether there is a problem with your revision}
% when embedding a single secret image, LDH performs slightly lower than other two methods. We consider that the scaling operations cause some loss of details inside the image. Furthermore, LDH shows its superiority when hiding multiple images. The quality of $S'$ generated by LDH will not be affected by the number of secret images because in LDH, the hiding and revealing processes of different secret images are independent, and the secret codes of different secret images will not affect each other. But


% quality of the stego image $C'$ generated by our LDH is significantly better than baselines in all three metrics when hiding a single image, including on the ImageNet and COCO datasets. Specifically, in terms of PSNR, our LDH achieves 5.924 dB and 3.852 dB improvement than the result for DDH and UDH respectively on the ImageNet dataset. We also provide 7.176 dB and 5.372 dB improvement respectively on the COCO dataset.


% In addition, according to Table \ref{table:performance}, we can see that the quality of $S'$ recovered by our LDH is slightly worse than that of $S'$ recovered by the other two methods, but we believe that the sacrifice of the recovery quality is made in exchange for a higher embedding rate. According to the experimental results, as the number of hidden images rises, the quality of $C'$ generated by our LDH decreases somewhat, but still reaches a comparable level. Unlike the $C$/$C'$ image pairs, the quality of the $S'$ recovered by LDH is not affected by the number of hidden images, and the recovery effect of hiding one and hiding many is the same. The experimental results of LDH in Table \ref{table:performance} are measured at a scaling factor of 4, which shows that when the cover image $C$ is full of secret images (i.e. 16 secret images are embedded), each $S'$ recovered by LDH has a high quality.

% One-to-many experiment results will be described in detail in the next subsection.

% \begin{table}
%     \centering
%     \caption{Performance comparison between DDH, UDH and our LDH. C denotes the cover/stego image pairs, and S denotes the secret/recovery image pairs. LDH-1 denotes hiding 1 image into the cover image, LDH-2 and LDH-4 are similar to it.}
%     \label{table:performance}
%     \begin{tabular}{cccccccc}
%     \toprule
%                             &        & \multicolumn{3}{c}{ImageNet} & \multicolumn{3}{c}{COCO}  \\
%     \hline
%                             & Method & APD$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$            & APD$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$         \\
%     \hline
%     \multirow{5}{*}{C}  & DDH    & 2.552   & 37.963    & 0.961               & 2.417   & 37.942    & 0.978            \\
%                             & UDH    & 2.031   & 40.035    & 0.979               & 2.121   & 39.746    & 0.981            \\
%                             & LDH-1  & \textbf{0.346}   & \textbf{43.887}    & \textbf{0.994}               & \textbf{0.292}   & \textbf{45.118}    & \textbf{0.996}            \\
%                             & LDH-2  & 0.657   & 41.188    & 0.987               & 0.572   & 42.185    & 0.989            \\
%                             & LDH-4  & 1.377   & 37.901    & 0.974               & 1.140   & 39.283    & 0.983            \\
%     \hline
%     \multirow{5}{*}{S} & DDH    & 2.261   & 39.055    & 0.991               & 1.956   & 39.614    & 0.989            \\
%                             & UDH    & 2.850   & 35.796    & 0.969               & 2.694   & 36.708    & 0.975            \\
%                             & LDH-1  & 3.809   & 33.169    & 0.951               & 4.263   & 31.514    & 0.939            \\
%                             & LDH-2  & 3.809   & 33.169    & 0.951               & 4.263   & 31.514    & 0.939            \\
%                             & LDH-4  & 3.809   & 33.169    & 0.951               & 4.263   & 31.514    & 0.939            \\
%     \bottomrule
%     \end{tabular}
% \end{table}

\textbf{Qualitative Results.} We exhibit some visualization results in Fig. \ref{fig:examples} to further show the superiority of our LDH. First, in the hiding phase, LDH brings the smallest perturbations for the cover images (see the column 2 in Fig. \ref{fig:examples}). The baselines are of global hiding, where the perturbations in the smooth area of the stego image can be easily detected, such as the perturbations in the sky. Specifically, DDH \cite{baluja2017hiding} may produce noise points in local areas; UDH \cite{zhang2020udh} generates a stego image with undesired horizontal stripes; MISDNN \cite{das2021multi} produces severe color distortion; and HCVS \cite{weng2019high} has obvious distortion at the edges of the secret images. Although LDH still produces horizontal stripes, we can avoid these stripes being easily found by selecting textured local areas for hiding. For example, in Fig. \ref{fig:jnd}, we use JND method \cite{wu2017enhanced} to determine more suitable local area (e.g., the woods) for carrying secret information, which achieves better quality of the stego images both subjectively and objectively.

% From Fig. \ref{fig:examples}, it can be observed that the difference between the cover and stego images in LDH is much smaller than those in other hiding schemes (Column 2, Fig. \ref{fig:examples}) during the hiding phase, which is consistent with the quantitative results. The distortion in the hiding phase of other schemes is distributed throughout the stego images and cases undesired blurring artifacts that are easily observed in the smooth regions of the stego images. Specifically, DDH \cite{baluja2017hiding} may produce noise points in local areas, UDH \cite{zhang2020udh} generates a stego image with undesired horizontal stripes, MISDNN \cite{das2021multi} produces severe color distortion, and Weng et al. \cite{weng2019high} has obvious distortion at the edges of the secret images. On the contrary, the stego image generated by LDH has almost invisible distortion only in the local region containing secret codes, the rest region is identical with the original cover image and thus has higher quality. Besides, as shown in Fig. \ref{fig:jnd}, using the JND method \cite{wu2017enhanced}, LDH is able to avoid embedding secret images into the smooth region of $C$, but rather into the texture-rich region that is least noticeable after adding noise, which further reduces the negative impact to the quality of the generated stego images.}

In the revealing phase, LDH still performs satisfactory. As shown in Fig. \ref{fig:examples}, we hide four different secret images in one cover image. From the revealed secret images we can see that LDH realizes the highest visual quality. By contrast, artifacts and colour distortions appear in the secret images revealed by other schemes. And these undesired distortions will become more seriously as the number of secret images increases (see Fig. \ref{fig:stego_quality}). Fortunately, our LDH is not bothered by this problem due to the characteristic of the local embedding.
%  To our best knowledge, this property is not possessed by any other deep hiding schemes.

We also illustrate the image quality comparison results of DDH \cite{baluja2017hiding}, UDH \cite{zhang2020udh} and our LDH under different embedding rates (from 1$\times$24 bpp to 6$\times$24 bpp) in Fig. \ref{fig:stego_quality} . The high quality of stego images is critical since it can better avoid manual or machine censorship. From Fig. \ref{fig:stego_quality:a} and \ref{fig:stego_quality:b},
%  and Table \ref{table:performance}
we can observe that for the baselines, the quality of the stego image gradually declines as the number of embedded images increases since more perturbations are introduced into the cover image to embed more images. Instead, our LDH still performs better at maintaining the quality of stego images, especially when hiding multiple secret images. In addition to the quality of stego images, Fig. \ref{fig:stego_quality:c} and \ref{fig:stego_quality:d} further show that in LDH, the quality of revealed secret images does not influenced by the number of embedded images. However, the corresponding visual quality of the baselines decreases seriously. From the whole Fig. \ref{fig:stego_quality}, we can conclude that LDH is much more suitable for high-capacity data hiding than these global ones.

% However, LDH still achieves a much better quality than DDH and UDH under the same embedding rate. Besides, for DDH and UDH, the average quality of the recovered secret images decreases as the number of embedded images increases. It is a general problem for global embedding methods. Low-quality recovery leads to meaningless secret sharing, which also limits the exploration of higher embedding rates in these works. In contrast, our local embedding strategy helps LDH avoid such problems, it can be seen that embedding multiple secret images does not affect the recovery quality in Table \ref{table:performance} and Fig. \ref{fig:stego_quality}.

% \lh{Fig. \ref{fig:examples} also illustrates a comparison between our LDH and the other methods during the revealing phase. As can be seen, when hiding four secret images, DDH \cite{baluja2017hiding} and Weng et al. \cite{weng2019high} will produce color distortion. For UDH \cite{zhang2020udh}, we can observe horizontal stripes over the revealed $S'$. For MISDNN \cite{das2021multi}, there exists severe blurring distortion and obvious color distortion. It is foreseeable that the recovery quality of these methods will be reduced to an unacceptable level if the embedding rate is further increased. Compared to these methods, our LDH can achieve the best average recovery quality, providing recovered secret images $S'$ with minimal error. Besides, as shown in Fig. \ref{fig:full_embed}, when concealing more images into one cover image, the revealing results of our LDH is almost the same as the revealing results when only embedding one image, i.e., all the recovered images are of high quality. To our best knowledge, this property is not possessed by any other deep hiding schemes.}


    % Images in the first row are the original cover image, the corresponding enlarged version of the region in red box, the original secret images, the corresponding enlarged version of the region in red box. The second to fifth rows show the results of every hiding scheme, with odd columns representing the hiding results and revealed results (PSNR or SSIM values are shown below the images) and even columns representing the deviations between the results and the ground truth. For better visualization, these deviations are magnified by a factor of 7.}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/experiment/jnd.pdf}
    \caption{Visual comparison of JND-guided position versus random position embedding the secret codes $S_e$. \textbf{Column 1:} The original cover image $C$. \textbf{Column 2:} The stego image $C'$ generated by random position embedding: $S_e$ is embedded into the red boxes. \textbf{Column 3:} Enlarge the parts in the red boxes. \textbf{Column 4:} The $C'$ generated under the guidance of JND: $S_e$ is embedded into the blue boxes. \textbf{Column 5:} Enlarge the parts in the blue boxes. The numbers below $C'$ indicates the SSIM value compared with $C$.}
    \label{fig:jnd}
\end{figure}

\begin{figure}[t]
    \centering
    \subfigure[]{\includegraphics[width=0.48\linewidth]{figs/analysis/cover_psnr.pdf}\label{fig:stego_quality:a}}
    \hfill
    \subfigure[]{\includegraphics[width=0.48\linewidth]{figs/analysis/cover_ssim.pdf}\label{fig:stego_quality:b}}
    \\
    \subfigure[]{\includegraphics[width=0.48\linewidth]{figs/analysis/secret_psnr.pdf}\label{fig:stego_quality:c}}
    \hfill
    \subfigure[]{\includegraphics[width=0.48\linewidth]{figs/analysis/secret_ssim.pdf}\label{fig:stego_quality:d}}

    \caption{Visual results of UDH, DDh, and LDH with different number of embedded images. (a) PSNR values of the cover/stego image pairs; (b) SSIM values of the cover/stego image pairs; (c) PSNR values of the secret/recovered image pairs; (d) SSIM values of the secret/recovered image pairs.}
    \label{fig:stego_quality}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/experiment/16imgs.pdf}
    \caption{Illustration of the maximum embedding rate (i.e., 16$\times$24 bpp) of LDH when $\omega$ is 4. Images in the yellow box are $C$, $C'$, $\times$15 magnified errors between $C'$ and $C$ from top to bottom. The 16 revealed images $S'$ are in the blue box.}
    \label{fig:full_embed}
    % \vspace{-10pt}
\end{figure}

\subsection{Impact of Hyper-parameters}
\textbf{Scaling Factor.} In our LDH, we use a scaling factor $\omega$ to determine the size of the compact secret codes, which also determines the upper bound of the embedding rate.
A larger  $\omega$ indicates a higher embedding rate.
However, a large $\omega$ also means extremely compact secret codes, which inevitably results in the loss of secret information and makes the recover of  high-quality secret images difficult. If the quality of the revealed secret image is too low, the corresponding hiding is meaningless and failed. We confirm this phenomenon in Table \ref{table:diff_scale}.
From Table \ref{table:diff_scale} and the results of LDH in Table \ref{table:performance}, we find that $\omega=4$ can balance the embedding rate and the quality of $S'$ better. As $\omega$ increases from 2 to 4, the quality of stego images is improved and the embedding rate reaches $16\times24$ bpp while sacrificing the quality of $S'$ about 6.24\%. The quality of $S'$ is acceptable when $\omega=4$ and the PSNR between the original and the revealed secret images is greater than 32 dB. Fig. \ref{fig:full_embed} illustrates the visual results of our LDH under $\omega=4$, where the revealing results of our LDH is almost the same as the revealing results when only embedding one image, i.e., all the recovered images are of high quality.
As we further increase $\omega$ from 4 to 8, the quality of $S'$ becomes unacceptable (the corresponding PSNR is only about 26 dB) although the theoretical embedding rate can be $64\times24$ bpp.
%  Given the results in Table \ref{table:performance} and \ref{table:diff_scale}, we mainly adopt $\omega=4$ in our experiments.


% Although the setting of $\omega=4$ sacrifices the quality of $S'$ somewhat, we still maintain the quality of $S'$ at an acceptable level (e.g., the PSNR is larger than 32 dB in Table \ref{table:performance}). This shows that we have achieved an extremely high embedding rate ($16\times24$ bpp) using our LDH. In addition, in Table \ref{table:diff_scale} and \ref{table:performance}, we also find that as $\omega$ decreases from 4 to 2, the quality of the stego images reduces by 15.43\% on average since the size of the secret code becomes larger. Table \ref{table:diff_scale} also shows the results when $\omega=8$. From the table, we observe that although the quality of the generated stego images is slightly improved, the quality of the revealed secret images is severely degraded (PSNR below 27 dB). Since the quality score is low, we recommend a scaling factor of 4 in our LDH.


% In the proposed deep hiding scheme LDH, the scaling factor is the special factor that affects the embedding rate. Since LDH requires that secret images must be embedded in different local regions of the cover image, the scaling factor determines the upper limit of the number of images that can be embedded in LDH (i.e., the square of the scaling factor). We train LDH with scaling factor of 2 and 4, and find that the final recovered secret image's ($S'$) quality is higher for scaling factor of 2 as shown in Table \ref{table:diff_scale}. In detail, with 4 secret images hidden, the PSNR of $S'$ with a scaling factor of 2 is 2.416 dB and 3.161 dB higher than the PSNR of $S'$ with a scaling factor of 4 on the COCO dataset and the ImageNet dataset, respectively. However, the quality of $C'$ obtained with a scaling factor of 4 is much higher than that with a scaling factor of 2, being 7.142 dB and 5.783 dB higher on COCO and ImageNet, respectively. For the deep hiding task, the quality of $C'$ determines whether the steganalysis can recognize the hidden secret information, and from this perspective, LDH performs best with a scaling factor of 4.

\begin{table*}[t]
    \centering
    \caption{The performance of our LDH under different scaling factor $\omega$.}
    \label{table:diff_scale}
    \resizebox*{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{3}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{$\omega$\textbf{=2, 1 image}}                                                                      & \multicolumn{6}{c|}{$\omega$\textbf{=8, 1 image}}                                                                       \\
        \cline{2-13}
                                 & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}               & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}                \\
        \cline{2-13}
                                 & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$  \\
        \hline
        COCO                     & 1.321             & 0.976            & 38.246           & 3.527             & 0.965            & 33.93            & 0.114             & 0.998            & 48.19            & 8.606             & 0.822            & 25.891            \\
        \hline
        ImageNet                 & 1.36              & 0.972            & 38.078           & 2.676             & 0.977            & 36.33            & 0.117             & 0.998            & 48.045           & 8.078             & 0.843            & 26.665            \\
        \hline
        \multirow{3}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{$\omega$\textbf{=2, 2 images}}                                                                     & \multicolumn{6}{c|}{$\omega$\textbf{=8, 2 images}}                                                                      \\
        \cline{2-13}
                                 & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}               & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}                \\
        \cline{2-13}
                                 & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$  \\
        \hline
        COCO                     & 2.608             & 0.947            & 35.288           & 3.527             & 0.965            & 33.93            & 0.228             & 0.996            & 45.182           & 8.606             & 0.822            & 25.891            \\
        \hline
        ImageNet                 & 2.666             & 0.949            & 35.186           & 2.676             & 0.977            & 36.33            & 0.234             & 0.996            & 45.033           & 8.078             & 0.843            & 26.665            \\
        \hline
        \multirow{3}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{$\omega$\textbf{=2, 4 images}}                                                                     & \multicolumn{6}{c|}{$\omega$\textbf{=8, 4 images}}                                                                      \\
        \cline{2-13}
                                 & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}               & \multicolumn{3}{c|}{\textbf{Cover/Stego pair}}                   & \multicolumn{3}{c|}{\textbf{Secret/Recovery pair}}                \\
        \cline{2-13}
                                 & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & APD$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$  \\
        \hline
        COCO                     & 5.34              & 0.88             & 32.141           & 3.527             & 0.965            & 33.93            & 0.454             & 0.992            & 42.177           & 8.606             & 0.822            & 25.891            \\
        \hline
        ImageNet                 & 5.381             & 0.889            & 32.118           & 2.676             & 0.977            & 36.33            & 0.468             & 0.991            & 42.028           & 8.078             & 0.843            & 26.665            \\
        \hline
    \end{tabular}}
\end{table*}

\begin{table}[t]
    \centering
    \caption{Image quality Results of the revealed images under different capacities of the revealing networks. The results are measured by the PSNR and SSIM values between the secret and revealed images.}
    \label{table:decoder}
    \begin{tabular}{@{}cccc@{}}
        \toprule
        Models & nhf=48 & nhf=64 & nhf=80\\
        \midrule
        PSNR & 31.382 & 32.537 & 33.169\\
        SSIM & 0.930 & 0.942 & 0.951\\
        \bottomrule
    \end{tabular}
\end{table}

\textbf{Model Capacity.} In deep hiding, DNNs have a powerful representation ability to encode image information into their parameters, which is the biggest advantage of deep hiding compared to traditional data hiding and is the key to achieve high embedding rate. Besides, we think that deep neural networks with a higher capacity can support a higher embedding rate. To confirm it, we test multiple networks of different scales. Specifically, we change the width of all layers in the revealing network to control the number of hidden features (nhf), and record the corresponding experimental results in Table \ref{table:decoder}. As we can observe from Table \ref{table:decoder}, a larger nhf (i.e., a wider revealing network) leads to higher PSNR and SSIM scores. Therefore, model capacity is critical for a high embedding rate in deep hiding.


% In deep hiding, DNNs have a powerful representation ability to encode image information into their parameters, which ensures the complete and high-quality recovery of the secret image. According to this viewpoint, a larger DNN can memorize more serviceable information, that is, a larger DNN can improve the quality of revealed images under the guidance of a suitable hiding strategy. To confirm it, we explore different widths of the revealing network in our LDH, and record the PSNR and SSIM between the secret and revealed images in Table \ref{table:decoder}. As we can observe from Table \ref{table:decoder}, a larger number of hidden features (nhf) (meaning a wider revealing network) leads to higher PSNR and SSIM. This proves that the model capability is critical for the high embedding rate in deep hiding.

\subsection{Robustness Analysis}
During the transmission of $C'$, $C'$ could be distorted by unavoidable channel noises or artificial perturbations (e.g., JPEG compression, rotation, and cropping). In this case, strong robustness allows hiding schemes more practical in the real world.
% can help avoid the loss of secret information in the real world.
% This is particularly important for digital watermarking (a common application of data hiding).
Next, we will show that our LDH can naturally resist local distortions, and can be further enhanced by adversarial training to resist global distortions.

% presenting the innate advantages and acquired learning of the proposed LDH.

\textbf{Local Distortions.} Due to the special local embedding strategy, LDH can resist local distortions, e.g., random crop. Existing global deep hiding schemes suffer from the weakness of low redundancy \cite{xiang2021peel} and the missing of any part of a stego image will lead to wrong recovery of the corresponding secret pixels.
However, the missing of a random part of the stego image in our LDH may not affect the revealing of the secret image since the secret code is embedded locally and randomly. Thus, it is still possible for LDH to reveal the complete secret image after the stego image has experienced some local distortions. And the more compact of the secret code (i.e., larger $\omega$), the higher the probability of the complete recovery is.

To show the innate robustness of LDH, we adopt a cropping operation to erase part pixels from stego images. In particular, after the cropping, we can fill the hole in the stego image with the corresponding part of the cover image (\textit{Cropout}), or directly fill the hole with 0 (\textit{Crop}). In Fig. \ref{fig:crop}, we use Crop and Cropout to process the stego images (the size of the cropped hole is $400\times400$). From Fig. \ref{fig:crop}, we can see the innate robustness of LDH against Crop and Cropout intuitively. The Crop and Cropout operations do not affect the revealing of the secret code in LDH if the cropped area and embedded area do not overlap. However, the global hiding schemes (e.g.,DDH \cite{baluja2017hiding} and UDH \cite{zhang2020udh}) are certainly unable to recover the complete $S'$ after the cropping operation.
%  We must admit it is still possible that the cropped and embedded areas overlap, but this probability is much small especially for a large $\omega$.
To better illustrate this case, we also show the examples of the overlapping (column 3 and column 7) in Fig. \ref{fig:crop}. The specific numerical results of PSNR after the cropping attacks are exhibited in Table \ref{table:crop}, in which we first divide the stego image into 16 disjoint blocks and each block is 256$\times$256 pixels, and then randomly select 1, 2 and 4 blocks for executing Crop or Cropout. From Table \ref{table:crop}, it is clear to observe that LDH is more robust to cropping attacks than the other two global schemes due to the much higher quality of the revealed secret images.
% According to Fig. \ref{fig:crop}, LDH has an inherent advantage in robustness to cropping attacks that other schemes don't have. As for the quantitative experiments, we first divide the stego image with a resolution of 1024*1024 into 16 patches with a resolution of 256*256, and then randomly select some of these blocks for Crop and Cropout attacks, and measure the quality of recovery by different methods. The results are shown in the Table \ref{table:crop}

% LDH hides the secret information in the local region of the cover image, therefore has better robustness against various forms of attacks (e.g., noise injection, random erasing, etc). The attack is performed on $C'$ as a whole, it actually has less impact on the regions containing secret information, so the recovery process is less affected compared to other schemes.

% For example, deep hiding has the weakness of low redundancy, where a single pixel of $C'$ is corrupted will result in a tiny area of $S'$ not being recovered \cite{xiang2021peel}. For a general deep hiding scheme, if $C'$ is subjected to a cropping attack during transmission, even if the scheme is trained to target the cropping attack, it eventually cannot achieve a good recovery. On the other hand, the proposed LDH benefits from the local embedding attribute, the embedded secret images are well recovered as long as the region of $C'$ containing secret information is not subject to cropping attacks. LDH has strong robustness to cropping without the need for specialized training, which makes it suitable for some multimedia data transmission scenarios.

% To verify the above conclusion, we test two cropping methods with different models: \textbf{Cropout}, which replaces a rectangular region of the container image with the corresponding region of the cover image, and \textbf{Crop}, which directly fills a rectangular region of the container image with 0.

% A quantitative comparison with other schemes is shown in the Table \ref{table:crop}.

\begin{table}[t]
    \centering
    \caption{The recovery quality results of DDH, UDH and our LDH after the suffering crop attacks. The results are measured by PSNR. The suffix number is the number of randomly cropped blocks.}
    \label{table:crop}
    \begin{tabular}{cccc}
        \toprule
        Method    & DDH    & UDH    & LDH     \\
        \hline
        Crop-1    & 23.699 & 21.573 & 30.863  \\
        Cropout-1 & 23.571 & 21.557 & 30.656  \\
        Crop-2    & 20.228 & 18.918 & 29.022  \\
        Cropout-2 & 20.217 & 18.814 & 29.843  \\
        Crop-4    & 17.225 & 16.509 & 26.059  \\
        Cropout-4 & 17.227 & 16.461 & 26.255  \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{figure*}[!t]
    \centering
    \resizebox*{\textwidth}{!}{
        \huge
        \begin{tabular}{ccccccccc}
            & Stego image                                                                             & Global schemes                                                                            & Ours-1 & Ours-2                                                                                       & Stego image                                                                             & Other                                                                                       & Ours-1 & Ours-2                                                                                         \\
    \begin{sideways}Cropout\end{sideways} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/C1.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/UDH_S1.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/LDH_S1_hit.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/LDH_S1.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/C2.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/UDH_S2.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/LDH_S2_hit.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Cropout/LDH_S2.png}}  \\
    \begin{sideways}Crop\end{sideways}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/C1.png}}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/UDH_S1.png}}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/LDH_S1_hit.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/LDH_S1.png}}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/C2.png}}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/UDH_S2.png}}    & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/LDH_S2_hit.png}} & \makecell*[c]{\includegraphics[width=0.30\linewidth]{./figs/experiment/Crop/LDH_S2.png}}
    \end{tabular}
    }
    \caption{Visualization of the recovery effect after Cropout and Crop attack on the stego image. The first four columns are attacked at the top left corner and the last four columns are attacked at a random position of the stego image. The size of the image is 1024$\times$1024 pixels and the size of the cropped region is 400$\times$400 pixels.}
    \label{fig:crop}
\end{figure*}

\textbf{Global Distortions.} Besides the local distortions, our LDH can also resist other common global distortions by targeted adversarial training \cite{zhang2020udh}. In the adversarial training, we add a noise layer between the hiding and revealing modules, which simulates possible distortions and processes $C'$. We then train $P$ and $R$ to identify the embedding regions and reveal desired secret images from the processed $C'$ respectively. In particular, we consider three different distortions here to verify the acquired enhancement of LDH: \textit{Dropout} (Dropout replaces each pixel of $C'$ with the corresponding pixel of $C$ with a certain probability. We set the probability to 0.3), \textit{Gaussian Blur} (short as Gaussian), and \textit{JPEG Compression} (short as JPEG). Then we use a Dropout layer, a Gaussian layer, and a JPEG layer to play the role of the noise layer in the adversarial training. Note that, we can only use one of the three noise layers to process $C'$ (specialized) or use all three layers to process $C'$ (combined).
% We can enhance the robustness based on a single distribution or on the combination of all distributions.

We evaluate the robustness of the vanilla models (i.e., no adversarial training) and the corresponding enhanced models, and show the results in Table \ref{table:robustness}. From Table \ref{table:robustness}, it is clear to observe that before the adversarial training, the vanilla model does not work facing all considered distortions since the quality of the revealed secret images is extremely low (PNSR $<$ 13 dB), which means the corresponding secret images are useless. However, after the adversarial training, the robustness of LDH has been significantly improved. For the specialized models, the PSNR of the revealed secret images under all three distortions is 2--3 times better than the vanilla model. In addition, the quality of the revealed secret images obtained by the combined model is slightly lower than that of the specialized models, but still at an acceptable level. The results of the combined model show a significant improvement over the vanilla model, with robustness to multiple distortions and stronger generalization ability.

% after adding the distortion layer to the vanilla model, the quality of $C'$ is nearly unaffected, but the quality of $S'$ drops very severely that it is even unusable. The specialized models have a much improved recovery effect compared to the vanilla model. Besides, the quality obtained by combined model against Dropout and Gaussian is somewhat degraded compared to the quality by specialized models, but this is acceptable. Because the results of combined model are significantly improved compared to those of the vanilla model, it can be assumed that the model is trained to be robust to multiple distortions and has a strong generalization capability.

% The models that will be tested for comparison include the vanilla model that is not specifically trained, the specialized models that are specifically trained for a particular distortion, and the combined model that is trained with a combination of various distortions. The specialized training models add a particular type of distortion to a portion of the training samples at each iteration. Similarly, when training a model combining various distortions, we divide a minibatch into several parts and add a different type of distortion to each part or no distortion at all, so that the training can converge faster and enhance the performance.

% % Similar to the cropping attack, LDH also has better robustness against other forms of attacks (e.g., noise injection, random erasing and so on). Since the attack is performed on the $C'$ as a whole, it actually has less impact on the regions containing secret information, so the recovery process is less affected compared to other schemes.

% In the experiments, we set the dropping out probability of Drop layer to $p=0.5$, the width of Gaussian kernel of Gaussian layer to $\sigma=2$, and the quality factor of JPEG layer $Q=50$. The quality of the container image and the recovered secret image generated by the above three models are tested at the scaling factors of 0.25 and 0.5, respectively. The experimental results are shown in table \ref{table:robustness}.

\begin{table*}[ht]
    \centering
    \caption{The visual quality results of stego images and secret images under different image distortions. ``Vanilla training'': training without distortions; ``Specialized training'': training with a single corresponding distortion; ``Combined training'': training with combined distortions. ``Original'' indicates that no image distortions are added during the experiments.}
    \label{table:robustness}
    \resizebox*{0.75\linewidth}{!}{
    \begin{tabular}{|c|ccccccccc|}
    \hline
    \multirow{3}{*}{\textbf{Distortion type}} & \multicolumn{9}{c|}{Stego}                                                                                                                                                                                                                      \\ \cline{2-10}
                                     & \multicolumn{3}{c|}{\textbf{Vanilla Model}}                                                         & \multicolumn{3}{c|}{\textbf{Specialized Models}}                                                   & \multicolumn{3}{c|}{\textbf{Combined Model}}                               \\ \cline{2-10}
                                     & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & \multicolumn{1}{c|}{PSNR$\uparrow$ }   & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & \multicolumn{1}{c|}{PSNR$\uparrow$ }   & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & PSNR$\uparrow$    \\ \hline
    Original                           & \multicolumn{1}{c|}{0.343}  & \multicolumn{1}{c|}{0.994} & \multicolumn{1}{c|}{43.928} & \multicolumn{1}{c|}{0.418}  & \multicolumn{1}{c|}{0.991} & \multicolumn{1}{c|}{42.766} & \multicolumn{1}{c|}{0.583}  & \multicolumn{1}{c|}{0.985} & 40.619 \\ \hline
    Dropout                     & \multicolumn{1}{c|}{0.336}  & \multicolumn{1}{c|}{0.993} & \multicolumn{1}{c|}{44.039} & \multicolumn{1}{c|}{0.413}  & \multicolumn{1}{c|}{0.991} & \multicolumn{1}{c|}{42.876} & \multicolumn{1}{c|}{0.588}  & \multicolumn{1}{c|}{0.987} & 40.562 \\ \hline
    Gaussian                    & \multicolumn{1}{c|}{0.344}  & \multicolumn{1}{c|}{0.993} & \multicolumn{1}{c|}{43.926} & \multicolumn{1}{c|}{0.474}  & \multicolumn{1}{c|}{0.990}  & \multicolumn{1}{c|}{41.878} & \multicolumn{1}{c|}{0.586}  & \multicolumn{1}{c|}{0.986} & 40.586 \\ \hline
    JPEG                        & \multicolumn{1}{c|}{0.344}  & \multicolumn{1}{c|}{0.994} & \multicolumn{1}{c|}{43.938} & \multicolumn{1}{c|}{0.557}  & \multicolumn{1}{c|}{0.987} & \multicolumn{1}{c|}{40.909} & \multicolumn{1}{c|}{0.585}  & \multicolumn{1}{c|}{0.986} & 40.597 \\ \hline
    \multirow{3}{*}{\textbf{Distortion type}} & \multicolumn{9}{c|}{Secret}                                                                                                                                                                                                                         \\ \cline{2-10}
                                     & \multicolumn{3}{c|}{\textbf{Vanilla Model}}                                                         & \multicolumn{3}{c|}{\textbf{Specialized Models}}                                                   & \multicolumn{3}{c|}{\textbf{Combined Model}}                               \\ \cline{2-10}
                                     & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & \multicolumn{1}{c|}{PSNR$\uparrow$ }   & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & \multicolumn{1}{c|}{PSNR$\uparrow$ }   & \multicolumn{1}{c|}{APD$\downarrow$ }    & \multicolumn{1}{c|}{SSIM$\uparrow$ }  & PSNR$\uparrow$    \\ \hline
    Original                           & \multicolumn{1}{c|}{3.667}  & \multicolumn{1}{c|}{0.957} & \multicolumn{1}{c|}{33.615} & \multicolumn{1}{c|}{4.477}  & \multicolumn{1}{c|}{0.934} & \multicolumn{1}{c|}{31.961} & \multicolumn{1}{c|}{9.960}   & \multicolumn{1}{c|}{0.834} & 25.431 \\ \hline
    Dropout                     & \multicolumn{1}{c|}{48.370}  & \multicolumn{1}{c|}{0.248} & \multicolumn{1}{c|}{12.420}  & \multicolumn{1}{c|}{7.564}  & \multicolumn{1}{c|}{0.885} & \multicolumn{1}{c|}{26.947} & \multicolumn{1}{c|}{11.685} & \multicolumn{1}{c|}{0.832} & 23.230  \\ \hline
    Gaussian                    & \multicolumn{1}{c|}{52.714} & \multicolumn{1}{c|}{0.309} & \multicolumn{1}{c|}{11.854} & \multicolumn{1}{c|}{5.047}   & \multicolumn{1}{c|}{0.917} & \multicolumn{1}{c|}{30.533} & \multicolumn{1}{c|}{9.787}  & \multicolumn{1}{c|}{0.856} & 24.927 \\ \hline
    JPEG                        & \multicolumn{1}{c|}{98.625} & \multicolumn{1}{c|}{0.187} & \multicolumn{1}{c|}{6.659}  & \multicolumn{1}{c|}{17.974} & \multicolumn{1}{c|}{0.737} & \multicolumn{1}{c|}{20.447} & \multicolumn{1}{c|}{16.956} & \multicolumn{1}{c|}{0.740}  & 20.711 \\ \hline
    \end{tabular}
    }
\end{table*}

% From this table, we can see that after adding the distortion layer to the vanilla model, the quality of the container image is nearly unaffected, but the quality of the recovered secret image drops very severely that it is even unusable. As for specialized models, the PSNR of the container images are 44.078dB, 44.947dB, 40.909dB, and that of the recovered images are 26.451dB, 30.413dB and 20.447dB, respectively. Compared to Dropout and Gaussian blurring, the model performs worse against jpeg compression. According to Zhang et al. \cite{zhang2020udh}, one possible reason is that the hiding process embeds the secret image into the high frequency region of the cover image, while jpeg compression has a greater effect on the high frequency region of the image. Besides, the quality of the container images obtained on combined model are similar, with PSNR around 40.58dB, while the quality of the recovered secret images are 23.23dB, 24.927dB and 20.711dB, respectively. The quality obtained by combined model against Dropout and Gaussian blurring is somewhat degraded compared to the quality by specialized models, but this is acceptable. Because the results of combined model are significantly improved compared to those of the vanilla model, it can be assumed that the model is trained to be robust to multiple distortions and has a strong generalization capability.


==> ieee copy/introduction.tex <==
\section{Introduction}\label{sec:introduction}
\IEEEPARstart{D}{ata} hiding or steganography is the art of hiding secret messages into innocent-looking cover objects such as images, videos or other computer files \cite{morkel2005overview,cheddad2010digital,anderson1998limits,bandyopadhyay2008tutorial,liu2021new,guan2022double}. This technology allows secret sharing in public channels without drawing suspicion to the transmission of the hidden information. A data hiding scheme usually consists of two phases, hiding and revealing. In the hiding phase, the secret message owner embeds the message into a cover medium (e.g., an image) to produce a stego medium, while preserving the fidelity of the cover medium. In the revealing phase, the receiver extracts the secret embedded message from the stego medium. In this paper, we concentrate on hiding and revealing secret message in images.
%  We concentrate on hiding secret messages within images in this paper.

During the evaluation of data hiding schemes, the embedding rate is one of the most important metrics to measure the efficiency of secret sharing, which can be quantified by bits per pixel (bpp). Many efforts have been made to improve the embedding rate. For example, HUGO \cite{pevny2010using} minimizes a suitably-defined distortion with a designed coding algorithm to increase the embedding rate. Unfortunately, such traditional data hiding schemes \cite{pevny2010using, chan2004hiding,tamimi2013hiding,li2007steganographic,raja2005secure,mckeon2007strange,denemark2015improving,li2014new,li2015strategy} usually have a low embedding rate, e.g., HUGO only achieves about 0.5 bpp. Such a low embedding rate indicates that HUGO can be only used to transfer short text messages. To the best of our knowledge, this is also a common problem for most traditional data hiding schemes \cite{chan2004hiding,tamimi2013hiding,denemark2015improving,li2014new,li2015strategy}, especially for frequency-domain based schemes \cite{li2007steganographic,raja2005secure,mckeon2007strange}.

% In related studies, message capacity (or embedding rate) is one of the most important metrics to evaluate the efficiency of secret sharing, which can be quantified by bits per pixel (bpp). Many efforts have been made to improve the embedding rate. For example, HUGO \cite{pevny2010using} tries to increases the embedding rate by minimizing a suitably-defined distortion with a designed coding algorithm. Unfortunately, the increase is very limited, and HUGO only achieves about 0.5 bpp on average. Such a low embedding rate means that HUGO can be only used to transfer short text messages. To the best of our knowledge, this is also a common problem for most traditional data hiding schemes \cite{chan2004hiding,tamimi2013hiding,denemark2015improving,li2014new,li2015strategy}, especially for frequency-domain based schemes \cite{li2007steganographic,raja2005secure,mckeon2007strange}.

Recently, deep learning techniques have been applied to data hiding (i.e., deep hiding), which hides and reveals secret messages using deep neural networks (DNNs) and can significantly improve the embedding rate. Baluja et al. \cite{baluja2017hiding} first leverage DNNs to achieve a high embedding rate, 24 bpp, by hiding a full-size image into another one. After that, more deep hiding schemes \cite{zhang2020udh,yu2020attention,zhang2019invisible,lu2021large} are proposed to reach a similar or higher embedding rate. For example, Zhang et al. \cite{zhang2020udh} proposed a deep hiding scheme that can hide three secret images into a cover image (i.e., $3\times 24$ bpp) by training three pairs of hiding and revealing networks.

% Recently, researchers start to apply deep learning technology to data hiding due to the outstanding performance of deep learning in other fields. Deep learning-based data hiding (short as deep hiding), uses deep neural networks (DNNs) to construct the hiding and revealing algorithms, which not only simplifies the construction but also significantly improves the embedding rate. Baluja et al. \cite{baluja2017hiding} first proposed to hiding a full-size image within another one using DNNs, increasing the embedding rate to an amazing level: 24 bpp. Inspired by this work, more high-capacity deep hiding schemes \cite{zhang2020udh,yu2020attention,zhang2019invisible,lu2021large} are proposed to reach a similar or a higher embedding rate (e.g., 72 bpp in \cite{zhang2020udh}). So far, deep hiding schemes have shown their superiority in improving the hiding performance, including increasing the embedding rate and revealing high-quality secret images \cite{yu2020attention,zhang2019invisible}. Besides, deep hiding can be also applied to more challenging tasks, such as light field messaging \cite{wengrowski2019light,tancik2020stegastamp}, and performs much better than traditional ways.

Existing deep hiding schemes have achieved a high embedding rate, which either improve the image quality of secret images \cite{yu2020attention,zhang2019invisible} or provide fancy functionalities such as hiding hyperlinks into an image \cite{tancik2020stegastamp}, light field messaging \cite{wengrowski2019light}. However, there is little analysis of why this happens and what affects the embedding rate. In this paper, we intend to answer two more fundamental questions: 1) \textit{why DNNs can greatly improve the embedding rate?} 2) \textit{can the embedding rate be further greatly improved?} and 3) \textit{Are there any trade-offs between the embedding rate and image quality?}.

% Although deep hiding has achieved great success, there is little analysis of why this happens, especially what causes the unprecedented high embedding rate. In this paper, we intend to answer three fundamental questions: 1) \textit{why DNNs can greatly improve the embedding rate?}, 2) \textit{can the embedding rate be further greatly improved?}, and 3) \lh{{\textit{how to trade-off embedding rate and image quality?}}}.

For the first question, we find that DNNs are trained to encode secret images into imperceptible codes that are further embedded into cover images. Such an efficient coding technique can effectively reduce the scale of the secret images and highly improve the embedding rates of the corresponding hiding schemes. With such insights, we address the second question by designing a novel Local Deep Hiding (LDH) and further increase the embedding rate to an amazing level, $16\times 24$ bpp. In particular, our LDH uses a carefully designed DNN to encode a full-size secret image into a small \textit{imperceptible compact secret code} that is the key to improving the embedment rate. The small imperceptible compact secret code is randomly embedded in to a local region of a cover image. Since the remaining pixels of the cover image can be used for hiding other secret images, our LDH can embed much more images than existing deep hiding schemes that embed a full-size secret image into all pixels of the cover image.

Our LDH consists of three DNNs: hiding, locating, and revealing networks. The hiding network converts a given secret image into a small imperceptible compact secret code (looks like a noise image of small size) that will be added to a random local region of a cover image to produce the corresponding stego image. The locating network identifies the positions of all embedded secret codes in the stego image and outputs a binary location map, with which the revealing network recovers all full-size secret images from the determined small local regions in the stego image. Our LDH also can complete the embedding and recovering for all secret images through the same hiding and revealing networks, instead of training multiple pairs of hiding and revealing networks. Experimental results show that our LDH can achieve a much higher embedding rate while preserving the quality of both the cover and secure images.

To answer the last question, we construct an experiment scenario of secret sharing and present an in-depth analysis from the perspective of the message receiver. In particular, we assume that the receiver can use different algorithms to enhance the quality of the revealed secret images. We measure the highest embedding rates that can be achieved by various deep hiding schemes when the quality reaches a certain threshold. We show that the embedding rates of deep hiding schemes varies with different quality threshold. And as the embedding rate increases, the quality of the results revealed by existing hiding schemes gradually decreases, while our LDH does not exhibit this phenomenon. Besides, the embedding rate of a deep hiding scheme may be increased if the receiver owns a powerful image restoration model to enhance the image quality of the secret images.

% A highly probable answer to the first question is that a high-capacity DNN can store redundant image information in its numerous parameters during its training phase. As we all know, DNNs have strong representation ability, and enough parameters allow them to fit arbitrary functions in theory. Therefore, we believe that when the DNNs are required to embed a secret image with the same or even more size within a cover image while keeping the visual quality of the cover image, the DNNs will automatically extract and remember some redundant information in images, which can effectively reduce the scale of the secret codes. Thanks to more efficient coding, a cover image can carry more secret information, i.e., a higher embedding rate.

% To answer the second question, we first analyze the drawback of current deep hiding schemes. After analyzing mainstream deep hiding schemes, we find that most of them try to a secret image into secret codes having the same size as the cover images. We think such a strategy is global since it will allocate the information of a secret image to all cover pixels. Although many deep hiding schemes have further increased the embedding rate on the basis of 24 bpp through code superimposition \cite{zhang2020udh} or encoding multiple image into the same codes \cite{baluja2019hiding,das2021multi}, \textit{the upper bound of global hiding is relatively limited because of the mutual interference between the secret codes of different secret images.}

% To break the upper bound of the embedding rate of the global hiding, we turn to local hiding strategy and design a novel Local Deep Hiding (LDH). Different from previous global ways, our LDH converts a secret image into more compact codes, whose size is much smaller than cover images' so that the codes can be embedded locally. In LDH, we no longer improve the embedding rate by superimposing different secret codes liking that in \cite{zhang2020udh}, but by embedding different secret images in different local areas of the cover image, avoiding the problem of the mutual interference between different secret codes. As results, we can hide up to 16 different images in a cover image, and the corresponding embedding rate comes to inconceivable 384 bpp.

% Our LDH consists of three DNNs: hiding, locating, and revealing networks. The hiding network is responsible for a secret image into imperceptible yet compact secret codes (look like a noise image of small size), which will be embedded in a random local area of the cover image. The remaining unoccupied areas in the cover image can be used for carrying the compact codes of other secret images. Considering the embedding area is random, we design a locating network to assist the revealing process. The locating network identifies the location of embedded secret codes by outputting a binary map, in which 1 means the corresponding stego pixel carries secret information, and 0 means the opposite. With the guidance of the binary map, we crop the local areas containing secret information from the stego image and feed them to our revealing network, which can recover all corresponding secret images. Since the secret codes of different secret images are generated and embedded independently, they will not interfere with each other during the hiding and revealing process so that we can ensure that all recovered secret images are of high quality. Moreover, according to our view on the first question, we implicitly force the revealing network to remember more extra image information besides the secret codes compared with previous global ways as we reduce the scale of the secret codes sharply in LDH.

% \lh{To answer the last question, we construct a secret sharing scenario and present an in-depth analysis from the perspective of the message receiver. In particular, we assume that the receiver can use different algorithms to enhance the quality of the revealed secret images, and measure the highest embedding rate that can be achieved by various deep hiding schemes when the quality reaches a certain threshold. We show that as the embedding rate increases, the quality of the results revealed by existing hiding schemes gradually decreases, while our LDH does not exhibit this phenomenon. Besides, our LDH performs most outstandingly in terms of embedding rate at the same level of revealed quality.}

We summarize our main contributions below:
\begin{itemize}
    \item We propose a novel Local Deep Hiding (LDH) scheme to encode secret images into small imperceptible compact secret codes and further significantly increase the embedding rate.
    % \item We propose an importance map module to detect the embedded location of the secret message and to guide the revealing process of the decoder.
    \item We propose a two-stage training strategy to enhance the performance of our LDH.
    \item We conduct extensive experiments to evaluate the superiority of our LDH.
    \item We present an in-depth study to quantitatively analyze the trade-off between the embedding rate and image quality.
\end{itemize}

The remainder of the paper is organized as follows: Section \ref{sec:related_work} introduce data hiding and related works. In Section \ref{sec:algorithm}, we specify the details of our proposed scheme. In Section \ref{sec:experimental_evaluation} evaluates our scheme under various system settings, followed by a quantitative analysis of the trade-off between the embedding rate and image quality. Section \ref{sec:conclusion} concludes this paper.

==> ieee copy/related_work.tex <==
\section{Background and Related Work}
\label{sec:related_work}
% Data hiding schemes conceal a secret message within a cover file without affecting its fidelity. Thanks to this characteristic, the secret message can be transferred through public channels without attracting any attention \lhc{the first two sentence should be also placed in Introduction}.
To facilitate the description of a data hiding scheme, we use $S$ and $C$ to represent a secret message and a cover image respectively. $\epsilon_1$ and $\epsilon_2$ are two hyperparameters. $D$ measures the difference between two given inputs. A data hiding scheme consists of two necessary algorithms:
    \begin{itemize}
        \item \textbf{Hiding algorithm} ($H$) embeds $S$ into $C$ without affecting the visual quality of $C$, and outputs a stego image $C'$ (i.e., $C'=H(C, S)$), which has $D(C',C)\leq\epsilon_1$;
        \item \textbf{Revealing algorithm} ($R$) reveals the embedded secret message from $C'$ as $S'=R(C')$ and needs to meet $D(S',S)\leq\epsilon_2$.
    \end{itemize}
% In order to meet the application requirements, the hidden data needs to affect the cover as little as possible, and it needs to ensure that the revealed result should be as consistent as possible with the original secret data. Specifically, visual differences in $c/c'$ and $s/s'$ pairs should be minimized.
The performance of a data hiding scheme is often measured by the number of bits a cover pixel can carry, i.e., bits per pixel (bpp). A higher numerical value of bpp means that the corresponding data hiding scheme has a higher message capacity (i.e., a higher embedding rate).
% Compared with traditional data hiding, recently proposed deep learning-based data hiding (i.e., deep hiding) has realized a much higher message capacity.

\subsection{Data Hiding of Low Embedding Rates}
Some data hiding schemes embed secret messages into frequency domain domains such as iscrete cosine transform (DCT) domain \cite{provos2003hide,fard2006new,attaby2018data}, discrete wavelet transform (DWT) domain \cite{reddy2009high,atawneh2017secure}, discrete Fourier transform (DFT) domain \cite{mckeon2007strange,ruanaidh1996phase} and integer wavelet transform (IWT) domain \cite{gulve2015image,kalita2019new}. But such frequency-domain data hiding schemes can only reach a low embedding rate, such as 2 bpp or lower.
%  There are many choices for the frequency domain, including
% Traditional low-embedding-rate data hiding schemes \lhc{are achieved by frequency domain based methods.} These methods hide secret data in
% discrete cosine transform (DCT) domain \cite{provos2003hide,fard2006new,attaby2018data}, discrete wavelet transform (DWT) domain \cite{reddy2009high,atawneh2017secure}, discrete Fourier transform (DFT) domain \cite{mckeon2007strange,ruanaidh1996phase} and integer wavelet transform (IWT) domain \cite{gulve2015image,kalita2019new}.
For example, Attaby et al. \cite{attaby2018data} proposed DCT-M3 algorithm, which uses modulus 3 of the difference between two DCT coefficients to embed two bits of the secret message. Atawneh et al. \cite{atawneh2017secure} applied a diamond encoding method to realize a DWT-based hiding scheme, enhancing the quality of the stego images. McKeon and Robert \cite{mckeon2007strange} proposed a DFT-based scheme that provides a sophisticated method for hiding data in movies. Kalita et al. \cite{kalita2019new} developed an IWT-based method that uses only high-frequency subbands to conceal secret messages for resisting steganalysis. Although frequency-based schemes often show good robustness against common interference operations (e.g., compression), but they are highly computational complexity and can only achieve limit embedding rates.

% These methods have complex embedding and revealing process and are less affected by rotating, scaling and compressing, thus have \lhc{better} security.
Instead, other data hiding schemes embed secret messaves into the spatial domain, such as
% \lhc{An effective data hiding system always aims to embed more secret information into the cover media, which helps reduce the likelihood of interception when sent over insecure channels.} Maintaining a higher embedding rate without sacrificing imperceptibility and security is an important challenge for data hiding. Traditional high-embedding-rate data hiding methods are achieved by spatial domain based techniques, which include
least significant bit (LSB) \cite{chan2004hiding,jung2015steganographic,sahu2020reversible}, pixel value differencing (PVD) \cite{mandal2022high,li2018steganography}, histogram shifting \cite{thodi2007expansion,tai2009reversible,xie2020adaptive}, expansion based \cite{tian2003reversible,gujjunoori2019difference}, multiple bit-planes \cite{kieu2009high,nyeem2017reversible}. These methods have higher embedding rates than frequency-domain based methods, but are usually less robust and less resistant to steganalysis \cite{fridrich2001reliable,dumitrescu2002detection,fridrich2004estimation,ker2004improved,ker2005general}. The spatial-domain methods perform pixel operations directly and thus usually have higher embedding rates (such as more than 2 bpp). Recent works also use deep learning techniques to improve the embedding rate. For example,
% Rapid developments in the field of artificial intelligence have prompted researchers to turn to deep learning-based data hiding.
Hayes et al. \cite{hayes2017generating} devised a GAN-based data hiding to enhance the quality of the stego image. Ghamizi et al. \cite{ghamizi2019adversarial} used deep neural networks and adversarial attacks to embed secret information into images and improves the embedding rate to some extent. Hu et al. \cite{hu2018novel} proposed a steganography without embedding (SWE) method, which uses a trained generator neural network model to generate the stego image based on a noise vector, to further improve the ability to resist detection algorithms. Ray et al. \cite{ray2021image} used a deep supervision based edge detector to embed more bits into the edge pixels. Tancik et al. \cite{tancik2020stegastamp} devised a new framework StegaStamp to realize message hiding and revealing in the physical world. However, these data hiding schemes with deep learning focused on embedding binary messages into cover images and also have low embedding rates.


% and successfully reveal it after decoding. These methods have higher resistance to some steganalysis, but have only very limit message capacity, i.e., low embedding rate. \lhc{specific value}

\subsection{Data Hiding of High Embedding Rates}
A higher embedding rate indicate that more secret messages can be delivered through the same cover image, increasing the effectiveness of secret sharing. Existing data hiding schemes of high embedding rates hide full-size images within images using DNNs, which can realize more than 24 bpp.
% some deep learning based hiding methods have been proposed.
According to the different model structures, we can classify these schemes into three categories: encoder-decoder structure \cite{baluja2017hiding,weng2019high,rahim2018end,zhang2019invisible,zhang2020udh,das2021multi}, generative adversarial network (GAN) structure \cite{zhang2019steganogan,meng2019steganography,yu2020attention}, and invertible neural network structure (INN) \cite{lu2021large,guan2022deepmih}.

\textbf{Encoder-Decoder Structure.} Since the data hiding and revealing processes correspond exactly to the encoding and decoding processes, encoder-decoder structure is suited for data hiding models.
%  Such schemes combine CNNs to learn data representation, and implement data hiding and revealing functions end-to-end.
For example, Baluja et al. \cite{baluja2017hiding} first designed a framework for hiding images within image, which uses a preprocessing network to embed the secret images into a cover image using a hiding network.
%  Weng et al. \cite{weng2019high} applied a similar technology to video steganography by utilizing temporal residual modeling.
% proposed DDH that hides a full-size image within another one (i.e., 24 bpp embedding rate) using an encoder-decoder framework.
% Rahim et al. \cite{rahim2018end} adopted a similar end-to-end framework to conceal a gray image into a color image, realized 8 bpp embedding rate. Zhang et al. \cite{zhang2019invisible} added adversarial training on the basis of encoder-decoder framework, also realized 8 bpp by hiding a gray image in the Y channel of a cover image in YCrCb color space. In addition, they added a steganalyzer to identify whether the generated stego images contain secret information, thus further improving the quality of hiding process.
Zhang et al. \cite{zhang2020udh} removed the preprocessing network and designed a framework for large-capacity data hiding, in which the encoding process of secret images is independent of the choice of cover images and the secret codes can be hidden in any cover image. They further trained three pairs of hiding and revealing networks to improve the embedding rate to 72 bpp.
% made the embedding process independent of cover images and further improve the embedding rate to 72 bpp by hiding three images in one cover image using three pairs of hiding and revealing networks.
Similarly, Das et al. \cite{das2021multi} proposed MISDNN, which adopts several pairs of preparing networks, hiding networks, and revealing networks to achieve multiple-image hiding.

\textbf{GAN Structure-Based.} In this type of deep hiding, both the hiding and revealing processes can be achieved by a specialized generator, while the discriminator is responsible for making the generated results as close as possible to the original ones.
%  It has brought up interesting data hiding schemes.
% Zhang et al. \cite{zhang2019steganogan} proposed a technique for hiding arbitrary binary data in images using GAN, which achieved a payload of 4.4 bpp.
Meng et al. \cite{meng2019steganography} adopted CycleGAN \cite{isola2017image} to achieve hiding images within images and improved the security of data hiding by adversarial training. Similarly, Yu et al. \cite{yu2020attention} also adopted GAN in deep hiding and further introduced an attention mechanism to improve the image quality.

\textbf{INN Structure.} This type of deep hiding schemes utilizes INNs \cite{dinh2014nice,dinh2016density} and shares parameters in the hiding and revealing networks instead of training two independent networks.
% , which makes the hiding and revealing more lighter.
% The most significant highlight of INN structure-based deep hiding is that the hiding and revealing networks share parameters, instead of training two independent networks.
% Recently, some deep hiding schemes have adopted an invertible neural network \cite{dinh2014nice,dinh2016density} framework, which can share the parameters in both hiding and revealing process.
Lu et al. \cite{lu2021large} used a INN to play both the hiding and revealing networks simultaneously and realized multiple-image hiding by concatenating multiple secret images in the channel dimension.
%  This operation of concatenating avoids training multiple networks for multiple-image hiding liking that in \cite{zhang2020udh}.
Guan et al. \cite{guan2022deepmih} developed an invertible hiding neural network (IHNN) that can be cascaded multiple times. When hiding multiple secret images, IHNN is able to guide the current image hiding based on the previous image hiding results.
% , thus making the hiding results more invisible.

Although existing deep hiding schemes improve the hiding performance significantly, especially the embedding rate, they still cannot fully answer the fundamental questions. To further analyze the functionality and improve the embedding rate, we will propose a novel local deep hiding scheme below.

% \subsection{Traditional Data Hiding}
% Traditional data hiding schemes rely on manually designed hiding rules, which not only requires researchers to have rich experience but also be hard to embed a large amount of secret information within a cover image.

% \textbf{Non-Adaptive.} \lhc{explain what is Non-Adaptive data hiding, and don't use steganography}. \lhc{I think it is not necessary to emphasize spatial domain and frequency domain.}
% \sout{Non-adaptive steganography is usually based on the spatial domain or the frequency domain.} Spatial domain-based schemes usually involve encoding at the level of the least significant bits (LSB), i.e., secret data is hidden in the LSB of the cover image. For example, Tian et al. \cite{tian2003reversible} proposed a difference expansion-based hiding method and realized 0.5 bpp when the PSNR score between the cover and stego images is about 37 dB. Thodi et al. \cite{thodi2007expansion} proposed a histogram shifting technique based on difference expansion as an alternative method for embedding location maps, which doubles the maximum embedding capacity (1 bpp). Chang et al. \cite{chang2008high} proposed a (7, 4) Hamming code-based data hiding method to achieve 1 bpp while keeping a high PSNR score between the cover and stego images. Similarly, Wang et al. \cite{wang2001image} developed a genetic algorithm to calculate the location where secret data will be hidden. Kieu et al. \cite{kieu2009high} proposed a multiple embedding strategy to embed secret bits horizontally and vertically, which increases the embedding rate to about 2 bpp. These methods are simple, but they also have drawbacks such as low robustness and weak resistance to steganalysis \cite{fridrich2001reliable,dumitrescu2002detection,fridrich2004estimation,ker2004improved,ker2005general}.

% Frequency domain-based steganography involves a series of transformation operations on an image. For example, JSteg algorithm \cite{provos2003hide} to hide the secret data by simply exchanging the LSBs of non-zero quantized discrete cosine transform (DCT) coefficients with secret messages bits. Similarly, Fard et al. \cite{fard2006new} combined the generic algorithm and DCT to better select the location of secret message embedding. Attaby et al. \cite{attaby2018data} proposed the DCT-M3 algorithm, which uses modulus 3 of the difference between two DCT coefficients to embed two bits of the secret message. In addition to DCT, some frequency domain steganography is based on other image transformation techniques. In \cite{reddy2009high}, the authors proposed high capacity and high security steganography using the discrete wavelet transform (DWT). Atawneh et al. \cite{atawneh2017secure} applied the diamond encoding scheme to the DWT steganography method, and reduced the distortion of the embedding to the stego image ($C'$). McKeon and Robert \cite{mckeon2007strange} proposed a discrete Fourier transform-based (DFT) scheme that provides a sophisticated method for hiding data in movies. In general, the frequency domain-based approaches can achieve high imperceptibility but only limited payload (i.e., low embedding rate).

% \textbf{Adaptive} \lhc{explain what is Adaptive Steganography} Adaptive steganography is a special case of the first two methods, which takes the statistical global features of the image before attempting to interact with the LSB or DCT coefficients. For example, HUGO algorithm \cite{pevny2010using} constrains the embedding changes to those parts of covers that difficult to model, such as textured or noisy regions. Raja et al. \cite{raja2008robust} proposed a robust image adaptive steganography using integer wavelet transform, which achieves better trade off between visual perceptivity and capacity.

% However, all these tranditional methods can only achieve low embedding rates. One of the reasons is that the hiding and revealing rules are manually designed and cannot automatically reduce the redundant information while embedding. Such a low embedding rate seriously limits the application of data hiding in large-scale secret sharing.

% \subsection{Deep Hiding}
% Different from traditional data hiding that heavily relies on researchers' experience, deep hiding uses DNNs to learn the hiding and revealing algorithms automatically, which not only simplifies the construction of data hiding schemes but also greatly improves the embedding rate. Existing deep hiding schemes can be divided into the following three categories according to the type of specific DNNs:

% \textbf{Autoencoder-based.} Hiding and revealing the secret information corresponds to the encoding and decoding process in an autoencoder respectively. Baluja et al. \cite{baluja2017hiding} first proposed a deep hiding scheme that hides a full-size image within another one (i.e., 24 bpp embedding rate) using two networks and then reveals the hidden image using another network. By utilizing temporal residual modeling, Weng et al. \cite{weng2019high} further applied this technology to video steganography. Rahim et al. \cite{rahim2018end} adopted a similar end-to-end framework to conceal a gray image into a color image, realized 8 bpp embedding rate. Zhang et al. \cite{zhang2019invisible} added adversarial training on the basis of the autoencoder, also realized 8 bpp by hiding a gray image in the Y channel of a cover image in YCrCb color space. In addition, they added a steganalyzer to identify whether the generated stego images contain secret information, thus further improving the quality of hiding process. Zhang et al. \cite{zhang2020udh} made the embedding process independent of cover images and further improve the embedding rate to 72 bpp by hiding three images in one cover image using three pairs of hiding and revealing networks. Similarly, Das et al. \cite{das2021multi} proposed MISDNN, which adopts several pairs of preparing networks, hiding networks and revealing networks to achieve multiple image hiding.

% \textbf{GAN-based.} Generative Adversarial Network (GAN) are used extensively in deep hiding. Both the hiding and revealing of secret information can be achieved by a specialized generator, while the discriminator is responsible for making the generated result as close as possible to the original. Zhang et al. \cite{zhang2019steganogan} proposed a technique for hiding arbitrary binary data in images using GAN, which achieved a payload of 4.4 bpp. Meng et al. \cite{meng2019steganography} concealed a full-size image into another one based on CycleGAN \cite{isola2017image} and improved the security of hiding by adversarial training. Similarly, Yu et al. \cite{yu2020attention} also adopted two pairs of generators and discriminators, introduced an attention mechanism to improve the image quality while achieving 24 bpp. Overall, the adversarial learning adopted in GAN-based models leads to greater robustness in deep hiding schemes.

% \textbf{Flow-based.} Recently, some deep hiding schemes \cite{lu2021large,guan2022deepmih} have adopted flow-based generative models. Unlike the previous two frameworks that require two or more networks, the flow-based generative model uses an invertible neural network \cite{dinh2014nice,dinh2016density} to accurately model the distribution of real data, where the revealing process is the inverse of hiding process. Lu et al. \cite{lu2021large} proposed an invertible steganography network (ISN) for image embedding and revealing using forward and backward propagation operations of a single invertible network. By concatenating multiple secret images in the channel dimension, ISN can hide multiple images simultaneously. Guan et al. \cite{guan2022deepmih} developed an invertible hiding neural network (IHNN) that can be cascaded multiple times. When hiding multiple secret images, IHNN is able to guide the current image hiding based on the previous image hiding results, thus making the hiding results more invisible.

% Although existing deep hiding schemes have greatly improved the embedding rate, these techniques simply use DNNs to improve the embedding rate without analyzing the reasons behind the improvement. In this paper, we intend to explore what improves the embedding rate in deep hiding and propose a new hiding scheme to reach a much higher embedding rate.
